How to Strategize Human Content Creation in the Era of GenAI?

Generative AI (GenAI) will have significant impact on content creation platforms. In this paper, we study the dynamic competition between a GenAI and a human contributor. Unlike the human, the GenAI's content only improves when more contents are created by the human over time; however, GenAI has the advantage of generating content at a lower cost. We study the algorithmic problem in this dynamic competition model about how the human contributor can maximize her utility when competing against the GenAI for content generation over a set of topics. In time-sensitive content domains (e.g., news or pop music creation) where contents' value diminishes over time, we show that there is no polynomial time algorithm for finding the human's optimal (dynamic) strategy, unless the randomized exponential time hypothesis is false. Fortunately, we are able to design a polynomial time algorithm that naturally cycles between myopically optimizing over a short time window and pausing and provably guarantees an approximation ratio of $\frac{1}{2}$. We then turn to time-insensitive content domains where contents do not lose their value (e.g., contents on history facts). Interestingly, we show that this setting permits a polynomial time algorithm that maximizes the human's utility in the long run. Finally, we conduct simulations that demonstrate the advantage of our algorithms in comparison to a collection of baselines.

==> HOLDER.tex <==
begin{proof}
The second part of the statement is proved immediately since when $|\agmgm(t)| = 0$ only negative utility can be accumulated so higher utility can be obtained by deviating to a strategy that stops playing.

The first part can be proved using the following claim. 
\begin{claim}
Consider a pure strategy which at round $t$ pulls an arm $i \notin \agmgm(t)$ when $|\agmgm(t)| \ge 1$ then it can replaced by a strategy which pulls the same arms before round $t$ and achieves at least the same utility. 
\end{claim}
\begin{proof}
Let the followed strategy be $S$ and the deviation strategy be denoted by $S'$. Note that if $S$ does not pull an arm at some round, then we consider it to be a pull from a dummy arm that leads to zero utility. By the above claim, either (1) no arm $\agmgm(t)$ is pulled again until the end of the horizon or (2) there exists some arm in $\agmgm(t)$ that was not pulled at round $t$ and is the first to be pulled from $\agmgm(t)$ after round $t$. 

For case (1), if we deviate to a strategy $S'$ which pulls the same arms as $S$ up to round $t-1$, then pulls some arm $j \in \agmgm(t)$ at round $t$ and then stops playing we would obtain a higher utility: 
\begin{align}
    u_{S'}(T) = u_S(t-1) + (\probc(\mu_j,\maxgenmu{t}) -c_j)  > u_S(t-1) + u_S(t:T) = u_S(T)
\end{align}
Note in the above that $u_S(t:T)<0$.

For case (2), let arm $j \in \agmgm(t)$ be the first arm in $\agmgm(t)$ to be pulled after round $t$ and let that round when it is pulled be  $t_j\leq T$. We will deviate to a strategy which pulls the same arms as $S$ up to round $t-1$, then pulls $j$ at round $t$ and then pulls the same arms pulled by $S$ from round $t_j+1$ to $T$ and then stops playing. It follows by the above that for a round $r \in \{t+1,\dots,T-(t_j-t)\}$ strategy $S'$ pulls the arm as pulled by $S$ in round $r+(t_j-t)$, see Figure \ref{fig:tape_1} for an illustration. Further, for a round $r$ denote by $\maxgenmu{r}$ and $\maxgenmu{r}'$ the maximum generative mean at that round $r$ under strategies $S$ and $S'$, respectively. Note that by construction of $S'$ we have $\maxgenmu{t}'=\maxgenmu{t}$. Moreover, let $\alpha_r$ and $\beta_r$  be the arms pulled at rounds $r$ under strategies $S$ and $S'$, respectively. Now we can lower bound the utility under $S'$ as follows
\begin{align}
    u_{S'}(T) & = u_S(t-1) + (\probc(\mu_j,\maxgenmu{t}) -c_j) + \sum_{r=t+1}^{T-(t_j-t)} [\probc(\mu_{\alpha_r},\maxgenmu{r}') - c_{\alpha_r}] \\ 
              & \ge u_S(t-1) + (\probc(\mu_j,\maxgenmu{t}) -c_j) + \sum_{r=t_j+1}^{T} [\probc(\mu_{\beta_r},\maxgenmu{r}) - c_{\beta_r}] \\ 
              & = u_S(t-1) + (\probc(\mu_j,\maxgenmu{t}) -c_j) + u_S(t_j + 1:T) \\ 
              & \ge  u_S(t-1) + u_S(t:t_j) + u_S(t_j + 1:T) \\ 
              & = u_S(T)
\end{align}
Note in the above that $u_S(t:t_j-1)<0$ by definition of $\agmgm(t)$ and therefore since $\probc(\mu_j,\maxgenmu{t}) -c_j \ge \probc(\mu_{a_t},\maxgenmu{t}) -c_{a_t}$ we must have $\probc(\mu_j,\maxgenmu{t}) -c_j \ge \probc(\mu_{a_t},\maxgenmu{t}) -c_{a_t} + u_S(t:t_j-1) = u_S(t:t_j)$. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.75\linewidth]{Pictures/tape_1.pdf}
    \caption{The arm pulls under strategy $S$ and the deviation strategy $S'$.}
    \label{fig:tape_1}
\end{figure}


\begin{figure}[h!]
    \centering
    \includegraphics[width=0.75\linewidth]{Figs/tape_1.png}
    \caption{The arm pulls under strategy $S$ and the deviation strategy $S'$.}
    \label{fig:tape_1}
\end{figure}


\begin{figure}[h!]
    \centering
    \includegraphics[width=0.75\linewidth]{Figs/tape_2.png}
    \caption{The arm pulls under strategy $S$ and the deviation strategy $S'$.}
    \label{fig:tape_1}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.75\linewidth]{Figs/tape_lemma_4_6_more_color.jpg}
    \caption{The arm pulls under strategy $S$ and the deviation strategy $S'$.}
    \label{fig:tape_1}
\end{figure}

\end{proof}
By (recursively) invoking the above claim on any strategy which does not pull an arm $i \notin \agmgm(t)$ when $|\agmgm(t)| \ge 1$ we can obtain a new strategy which achieves at least the same utility that always pulls arms from $\agmgm(t)$.  
\end{proof}

==> HOLDER_2.tex <==
\SE{seperate seperate seperate}

This further implies that the maximum generative mean will be:
\begin{align}
    \maxgenmu{t} \ge \mu - g(p^*) = \mu - g(\frac{10}{7}) = 0.9 - (0.7 - 0.35 \times \frac{10}{7} ) = 0.9 - 0.2 = 0.7 
\end{align}

Let $\max\limits_{i \in [k]} \frac{\gamma}{1-\gamma^{D_i}} \cdot (\gamma + \gamma^{D_i}) = p'$. Note that $p' < p^*$ by construction. The maximum value for the generative mean under delay non-violating pulls would be $\mu - g(p') < 0.7$. 
\SE{separate separate separate separateseparate} 

 
The first $k$ arms have the same mean $\mu_i=\mu=0.9$ whereas the last arm has a mean $\mu_0 =0.1$. Further, for all arms the cost is set to $c=0.6$. 
%Note that the above link function satisfies our assumed properties of continuity and monotonicity in the mean. 
As a reminder the generative mean for an arm $i$ is 
\begin{align}
    \genmu{i}(t)     & = \mu_i - g_i(\bar{N}_i(t-1)) \\ 
    \text{where} \ \ % & N_i(t-1) = \sum_{s=1}^{t-1} \indic[b_s=i] \gamma_i^{t-s} \\ 
    & \pullsh{i}(t-1) =  \sum_{r = 1}^{t-1} \gamma_i^{t-r} \times \mathbb{I} (b_r = i) 
\end{align}
For our reduction we will set 
\begin{align}
    g_i(x) = g(\lambda_i x) 
\end{align} 
where $\lambda_i >0$ is to be set according to the delay value $D_i$ and $g(.)$ is a function shared by all arms. The function $g_(.)$ is set equal to the following: 
\begin{align}\label{eq:def_p_inv}
g(n) =
\begin{cases} 
          0.7 - 0.35 n & \text{if } n \leq 2 \\
          0 & \text{if } n >2 
\end{cases}
\end{align}

Since the AI always pulls the arm with the maximum generative mean, therefore $\maxgenmu{t} \ge \max\limits_{i \in [k]} \genmu{i}(1)=\mu_1-g_i(0) =0.9 - (0.7-0)=0.2$. 

%We set $\probc(\mu_0,\Tilde{\mu})-c \leq \nu_0, \ \forall \Tilde{\mu} \ge \max\limits_{i \in [k]} \genmu{i}(1)$ \SE{here}. On the other hand, we will set $\probc(\mu,\Tilde{\mu}) -c > \nu_0 , \forall \Tilde{\mu}$. 

==> HOLDER_3.tex <==
\section{Proofs for Section \ref{sec:discounted}} \label{app:discounted_proofs}
\subsection{Hardness Proofs for Subsection \ref{subsec:discount_hardness}}
\cite{basu2019blocking} define the blocking bandits problem and shows that it is NP-hard to maximize the rewards even when all of the means are known. In blocking bandits, each arm $i \in \arms$ has a mean $\mu_i$ and additionally has associated with it a delay $D_i \ge 1$. If arm $i$ is pulled at round $t$ then it cannot be pulled again until at least round $t+D_i$, i.e. for $D_i-1$ consecutive rounds we cannot pull arm $i$. Given that, suppose we want to pull arms through the horizon to maximize the accumulated expected rewards, i.e. solving the following maximization problem: 
\begin{align}
    \maxreward:
    & \max_{b_1,b_2,\dots,b_T} \sum_{t=1}^T \mu_{b_t} \\ 
    & \text{s.t. each arm being pulled such that its delay $D_i$ is not violated}
\end{align}
 We will call the above problem \maxreward{}. 

\paragraph{Example:} To illustrate the problem consider the example below with delay values for arms $1,2$ and $3$. Then a feasible solution to the given example would be $3\ 1\ 2\ 1\ 3\ 1\ 2\ 1\ $
\begin{table}[h!]
    \centering
    \begin{tabular}{c}
       $D_1=2$\\
       $D_2=4$\\
       $D_3=4$\\
    \end{tabular}
    \caption{Example}
    \label{tab:my_label}
\end{table}

A simple instance of \maxreward{} for blocking bandits was shown to be NP-hard in \cite{basu2019blocking} as shown in the theorem below. 
\begin{theorem}[\cite{basu2019blocking}]\label{th:blockingMAB_is_np_hard}
Suppose that we have $k+1$ arms where $k$ many arms have a mean of $1$ and a delay value $D_i$ with $\sum_{i=1}^k \frac{1}{D_i}=1$ except for one arm of mean $0$ and delay $1$, then deciding if \maxreward{} has a solution of value of at least $T$ is NP-complete. 
\end{theorem}
We will use this instance to construct a reduction to our problem of the human maximizing utility given the AI selects the arm with the maximum generative mean in each round where the number of samples fed into the generative mean are discounted by some factor. Note that we will refer to the $K$ arms with mean $1$ as the first $K$ arms and the arm of mean $0$ as the last arm. Note that our proofs actually show that the decision version of our problem is NP-complete but NP-hardness follows straightforwardly based on that. 

The proof of theore



Now we will show that even if all of the arm have the same shrinkage function $g_i(.)=g(.)$ in the generative mean then the problem still remains NP-hard. 


We restate the theorem and give its proof
\begin{restatable}{theorem}{NPhardsamegamma}\label{th:NP_hard_same_gamma}
Even when all of the arms have the same cost $c$ and the same discount factor $\gamma$ the problem of finding a pure optimal strategy for the human is NP-hard. 
\end{restatable}
\begin{proof}
\SE{begin}
Now, we go through the details of the reduction. We will reduce the special instance of \maxreward{} from Theorem \ref{th:blockingMAB_is_np_hard} to the problem of finding a pure optimal strategy. Given a \maxreward{} instance with a horizon of value $T$ then we set the horizon value for our problem to value $T+1$. We call the $k$ arms with non-trivial delay values ($D_i \ge 2$) and mean $1$ the \emph{first $k$ arms}. Similar to the \maxreward{} instance we will have $k+1$ arms. We refer to the first $k$ arms when we say $i \in [k]$ instead of $i \in [k+1]$ and the last arm will have index $k+1$. The means of the first $k$ arms is set to the same value of $\mu=0.9$ whereas the last arm will have a value of $\mu_{k+1}=0.1$. Further, all arms have the same cost of $c=0.6$.   

We start by showing that a discount factor of $\gamma = \frac{1}{2}$ is sufficient to make the discounted number of samples strictly higher whenever the delay value is violated for an arm with a delay $D_i \ge 2$ in our reduction. 
We start with the following claim
\begin{claim}\label{cl:nbar_lower_bound}
If a pull violates the delay rule for an arm $i$ at round $t$, then we have:
\begin{align}
    N_i(t) \ge \gamma + \gamma^{D_i}
\end{align}
\end{claim}
\begin{proof}
Suppose the pull violates the delay rule at round $t$ then it must be the case that arm $i$ was pulled at least $D_i$ rounds before $t$. This means that the smallest value for the discounted number of samples will be:
\begin{align}
    N_i(t) \ge  \gamma + \gamma^{D_i} 
\end{align}
See Figure \ref{fig:viol_delay} for an example. 
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.75\linewidth]{Pictures/viol_delay.pdf}
    \caption{Example showing the smallest value for the discounted number of samples of an arm $i$ if its delay value is violated.}
    \label{fig:viol_delay}
\end{figure}
\end{proof}
Further, if the delay is never violated then we can establish an upper bound on the discounted number of samples as shown in the following claim
\begin{claim}\label{cl:nbar_upper_bound} 
If the delay rule for an arm $i$ is not violated then the discounted number of samples at any round $t$ is at most   
\begin{align}
    N_i(t) \leq \gamma \cdot \frac{1}{1-\gamma^{D_i}}
\end{align}
\end{claim}
\begin{proof}
If we are at round $t$ and the pulls for arm $i$ did not violate the delay then the highest value for the discounted number of samples would be as follows (see Figure \ref{fig:respect_delay} for an illustration): 
\begin{align}
    N_i(t) & \leq \gamma + \gamma^{D_i+1} + \gamma^{2D_i+1} + \gamma^{3D_i+1} + ... \\ 
                 & = \sum_{\ell=0}^{\infty} \gamma^{D_i \ell + 1} \\
                 & = \gamma \cdot \frac{1}{1-\gamma^{D_i}}
\end{align} 
 \begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{Pictures/respect_delay.pdf}
    \caption{Example showing the upper bound for the discounted number of samples of an arm $i$ if its delay value is violated.}
    \label{fig:respect_delay}
\end{figure}
\end{proof}
We want to set $\gamma$ to a value such the resulting discounted number of pulls for an arm when violating its delay is strictly higher than the discounted number of pulls when its delay is not violated. To do that based on the two previous claims it is sufficient to satisfy the following inequality 
\begin{align}
    \gamma \cdot \frac{1}{1-\gamma^{D_i}} < \gamma + \gamma^{D_i}   \label{eq:discount_ineq}
\end{align}
The following claim shows that this can be done by simply setting $\gamma=\frac{1}{2}$ as stated earlier. 
\begin{claim}
If $\gamma =\frac{1}{2}$ then for any arm $i$ with $D_i\ge 2$ we have
\begin{align}
    \gamma \cdot \frac{1}{1-\gamma^{D_i}} < \gamma + \gamma^{D_i}   \label{eq:discount_ineq}
\end{align}
\end{claim}
\begin{proof}
By Lemma \ref{lemma:bound_f_gamma_D} setting $\gamma=\frac{1}{2}$ would satisfy the inequality. 
\end{proof}

With $\gamma=\frac{1}{2}$ we can write the following fact.
\begin{fact}\label{fact:discounted_sep}
For any arm $i \in [k]$ with $D_i \ge 2$ if at round $t-1$ the delay rule was violated then $N_i(t-1) \ge \gamma+\gamma^{D_i} > \frac{\gamma}{1-\gamma^{D_i}}$. On the other hand, if the delay rule was not violated at any round up to and including $t-1$ then we have $N_i(t-1) \leq  \frac{\gamma}{1-\gamma^{D_i}} < \gamma+\gamma^{D_i}$. 
\end{fact}


Now we complete the details of the reduction, the generative mean for an arm $i$ is 
\begin{align}
    \genmu{i}(t)     & = \mu_i - g_i(N_i(t-1)) 
    %\\ 
    %\text{where} \ \ % & N_i(t-1) = \sum_{s=1}^{t-1} \indic[b_s=i] \gamma_i^{t-s} \\ 
    %& \pullsh{i}(t-1) =  \sum_{r = 1}^{t-1} \gamma_i^{t-r} \times \mathbb{I} (b_r = i) 
\end{align}
Note that since $\gamma=\frac{1}{2}$, the highest discounted number of samples will be $\frac{\gamma}{1-\gamma} =1$. For the last arm $g_{k+1}(n)=0.1-0.1n$. On the other hand, for the first $k$ arms we set 
\begin{align}
    g_i(x) = g(\lambda_i x) \ \forall \in [k]
\end{align} 
where $\lambda_i >0$ is to be set according to the delay value $D_i$ and $g(.)$ is a function shared by all of the first $k$ arms. The function $g(.)$ is set equal to the following: 
\begin{align}\label{eq:def_p_inv}
g(n) = 0.7 - 0.35 n 
\end{align}


Let $p^*=\frac{10}{7}$. Now for any $i \in \arms$ we will set $\lambda_i$ as follows: 
\begin{align}
    \lambda_i = \frac{p*}{\gamma + \gamma^{D_i}}
\end{align}
This implies that if the delay rule for an arm $i$ is violated then in the next round we have $\lambda_i N_i(t) \ge p^*$, see Figure \ref{fig:lambda_illust} for an illustration.  

Based on the above, similar to Fact \ref{fact:discounted_sep} the value of the maximum generative mean will exceed a threshold if the delay rule is violated in the first $k$ arms. 
\begin{fact}\label{fact:discounted_sep_genmu}
For any arm $i \in [k]$ with $D_i \ge 2$ if at round $t-1$ the delay rule was violated then $\genmu{i}(t) \ge \genmuu = 0.7$. On the other hand, if the delay rule had not violated at any round up to and including $t-1$ then we have $\genmu{i}(t) \leq  \genmul < \genmuu$ where $\genmul= 0.9 - g(\max\limits_{i \in [k]} \frac{p^*}{\gamma + \gamma^{D_i}} \frac{\gamma}{1-\gamma^{D_i}})$. 
\end{fact}
\begin{proof}
If the delay is violated at round $t-1$ for an arm $i \in [k]$ then we have in the next round $t$
\begin{align*}
    \genmu{i}(t) & = \mu_i - g_i(N_i(t-1)) \\ 
                 & \ge \mu_i - g( \lambda_i \cdot (\gamma+\gamma^{D_i})) && \text{(by Fact \ref{fact:discounted_sep})}\\
                 & = 0.9 - g(\frac{10}{7}) && \text{($p^*=\frac{10}{7}$)}\\ 
                 & = 0.9  - (0.7 - 0.35 \times \frac{10}{7}) \\ 
                 & = 0.9 - 0.2  \\
                 & = 0.7 \\ 
                 & = \genmuu 
\end{align*} 
On the other hand if the delay rule is not violated then the maximum possible value given to the function $g(.)$ can be 
\begin{align}
    \max\limits_{i \in [k]} \lambda_i \frac{\gamma}{1-\gamma^{D_i}} = \max\limits_{i \in [k]} \frac{p^*}{\gamma + \gamma^{D_i}} \frac{\gamma}{1-\gamma^{D_i}} < p^*
\end{align}
Therefore, based on the definition of $\genmul$ in the fact, we will always have $\genmu{i}(t) \leq  \genmul < \genmuu$.
\end{proof}

For all values of $0 \leq \mu_1,\mu_2 < 0.9$, we set the link function $\probc$ to a simple linear form\footnote{Note that by construction all of the mean values will be in $[0,1]$. Further, we will complete the definition of $\probc$ if $\mu_1 \ge 0.9$ or $\mu_2 \ge 0.9$ such that it is monotonic.}
\begin{align}
    \probc(\mu_1,\mu_2) = \frac{1+(\mu_1-\mu_2)}{2}
\end{align}

Note that by our choice for the shrinkage functions, the AI will always choose an arm from the first $k$ set since it is straightforward to show that $\maxgenmu{t} \ge \genmu{i}(t) \ge 0.2 > 0.1 \ge \genmu{k+1}(t) , \ \forall i \in [k]$ and $\forall t \in [T+1]$. Therefore, we can upper bound the utility of the last arm of mean $\mu_{k+1}$
\begin{align}
    \probc(\mu_{k+1},\maxgenmu{t}) - c \leq \frac{1+(0.1-0.2)}{2} - 0.6 = -0.15 < 0 
\end{align}
Therefore, the last arm always gives negative utility. 

%\SE{begin}
%Let $\theta(\mu) =  \frac{1+(\mu-\genmul)}{2}$. Note that $\theta(0.9)>0.6$.  

%Based on this if we pull an arm from the first $k$ set when the delay rule has been violated for any of them the utility we will gain will be
 We will now set the value for link function when the first argument $0.9 \leq \mu_1 \leq 1.0$ 
\begin{align}
    \probc(\mu_1,\mu_2) = \begin{cases} 
         \frac{1+(\mu_1-\mu_2)}{2} & \text{if } \mu_2 \ge  \genmul \\
         \frac{1+(\mu_1-\genmul)}{2} & \text{if } \mu_2 <  \genmul 
\end{cases}
\end{align}
If the second argument $0.9 \leq \mu_2 \leq 1$ and $\mu_1<0.9$ then we simply calculate $\probc(\mu_1,\mu_2)=1-\probc(\mu_2,\mu_1)$. 

From the above we can now separate the utility we gain from the first $k$ arms based on whether we violated their delay rule or not 
\begin{fact}\label{fact:seperate_util}
If the delay rule for any arm arm $i \in [k]$ with $D_i \ge 2$ is violated at round $t-1$ then the utility at the next round will be at most $0$. On the other hand, if the delay rule is not violated then we can obtain a maximum utility of exactly $\theta-c>0$ where $\theta=\frac{1+(0.9-\genmul)}{2}$.  
\end{fact}
\begin{proof}
If the delay rule is violated then by Fact \ref{fact:discounted_sep_genmu} it follows that the utility will be at most $\frac{1+(0.9-\genmuu)}{2}-0.6=\frac{1+(0.9-0.7)}{2}-0.6=0$. 

On the other hand, if the delay rule is not violated then pulling one of the first $k$ arms we can obtain a utility of $\frac{1+(0.9-\genmul)}{2}-0.6=\theta-0.6$. Since $0.6=\frac{1+(0.9-0.7)}{2} = \frac{1+(0.9-\genmuu)}{2} < \frac{1+(0.9-\genmul)}{2} = \theta$, therefore we have $\theta-0.6=\theta-c>0$. 
\end{proof}








\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{Pictures/lambda_scaling.pdf}
    \caption{The figure shows how when the delay value is violated for any arm $i$ its coefficient $\lambda_i$ would lead to $\lambda_i N_i(t) \ge p^*$.}
    \label{fig:lambda_illust}
\end{figure}

Now that we have given the details of the reduction. The following lemma is immediate
\begin{lemma}
The human can obtain a utility value of $(\theta-c) \cdot (T+1)$ if and only if he always pulls an arm from the set of first $k$ arms without violating their delay value except possibly at the last round $T+1$. 
\end{lemma}
\begin{proof}
Suppose the human violates the delay for some arm $i$ in the first $k$ set at a round $t \leq T$ then it follows that in the next round the highest utility that can be obtained is zero by Fact \ref{fact:seperate_util} and therefore the highest utility throughout the horizon will be $(\theta-c) \cdot (T-1)$. 

Now suppose that only arms from the first $k$ set are pulled without violating the delay rule in the first round $T$ rounds, then it follows that the utility will be $(\theta-c) \cdot (T+1)$. 
\end{proof}
By the previous lemma it follows that given a \maxreward{} instance of Theorem \ref{th:blockingMAB_is_np_hard} is a YES instance if and only if the human can obtain a utility of value $(\theta-c) \cdot (T+1)$ in our reduction. 
\end{proof}

\SE{BEGIN BEGIN BEGIN} 
Now we state the following theorem and give its proof 
\begin{restatable}{theorem}{NPhardsameshrinkage}\label{th:NP_hard_same_shrinkage}
Even when all of the arms have the same cost $c$ and the same shrinkage function $g(.)$ the problem of finding a pure optimal strategy for the human is NP-hard.  
\end{restatable}
\begin{proof}
We will follow a reduction similar to the previous of Theorem \ref{th:NP_hard_same_gamma}. The difference is that all arms will have the same shrinkage function $g(.)$ but the discount factor for the first $k$ arms will be will different and set according to the delay value $D_i$. 

The following two claims follow from Claims \ref{cl:nbar_lower_bound} and \ref{cl:nbar_upper_bound}, they are simply restated for different values of $\gamma_i$. 
\begin{claim}\label{cl:lower_bound_discount}
If a pull violates the delay rule for an arm $i$ at round $t$, then we have:
\begin{align}
    \bar{N}_i(t) \ge \gamma_i + \gamma_i^{D_i}
\end{align}
\end{claim}

\begin{claim}\label{cl:upper_bound_discount} 
If the delay rule for an arm $i$ is not violated then the discounted number of samples at any round $t$ is at most   
\begin{align}
    \bar{N}_i(t) \leq \gamma_i \cdot \frac{1}{1-\gamma_i^{D_i}}
\end{align}
\end{claim}




Let $g_u(\gamma,D) =  \gamma + \gamma^{D}$. Then it is clear that $g_u(.,D)$ is decreasing in $D$. Let $D_{\max} = \max_{i \in [K]} D_i$ then for the arms with delay $D_{\max}$ we set $\gamma_i=\gamma_{\max}=\frac{1}{2}$. For the other arms we will choose $\gamma_i \in (0,\frac{1}{2}]$ such that $\gamma_i + \gamma_i^{D_i} = \frac{1}{2} + \frac{1}{2^{D_{\max}}}$. This is possible since $g_u(\frac{1}{2},D_i) > g_u(\frac{1}{2},D_{\max}) = \frac{1}{2} + \frac{1}{2^{D_{\max}}}$ since $D_i < D_{\max}$ and since $\lim\limits_{\gamma_i \to 0^{+}}  g_u(\gamma_i,D_i) = 0 < g_u(\frac{1}{2},D_{\max})$. Since $g_u(\gamma,D_i)$ is continuous there must exist some value in $\gamma \in (0,\frac{1}{2}]$ such that $\gamma_i + \gamma_i^{D_i} = \frac{1}{2} + \frac{1}{2^{D_{\max}}}$. 

Setting $\gamma_i$ to such values would lead the discounted number of samples to be separated into two disjoint intervals based on whether the delay was violated as illustrated in Figure \ref{fig:diff_gamma} and proved in the following claim. 
\begin{claim}
If the arms $i \in \arms$ are pulled without violating the delay up to round $T$ then $\forall t\in [T+1]: \max_{i \in \arms} \bar{N}_i(t) <  \frac{1}{2} + \frac{1}{2^{D_{\max}}}$ whereas if the delay is violated in any round up to and including $T$ then there exists at least one round $t \in [T+1]$ such that $\max_{i \in \arms} \bar{N}_i(t) \ge \frac{1}{2} + \frac{1}{2^{D_{\max}}}$. 
\end{claim}
\begin{proof}
If we do not violate the delays then for any arm $i$ by Claim \ref{cl:upper_bound_discount} we have
\begin{align}
    \bar{N}_i(t) & \leq \gamma_i \cdot \frac{1}{1-\gamma_i^{D_i}} \\ 
                 & < \gamma_i + \gamma_i^{D_i}  && \text{(by Lemma \ref{lemma:bound_f_gamma_D} and since $\gamma_i \in (0,\frac{1}{2}]$)} \\
                 & = \frac{1}{2} + \frac{1}{2^{D_{\max}}} && \text{(by construction of the values $\gamma_i$)}
\end{align}
The second part of the claim follows by construction and Claim \ref{cl:lower_bound_discount}.
\end{proof}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Pictures/diff_gamma.pdf}
    \caption{For any arm, once the delay is violated the discounted number of pulls will be at least $\frac{1}{2}+\frac{1}{2^{D_{\max}}}$.}
    \label{fig:diff_gamma}
\end{figure}

Now we set the values $\probc(.,.)$ for the first $k$ arms. 
\begin{align}
    \probc(\mu,\mu-g(\bar{N}_i(t))) = \theta' \ \ \text{if $\bar{N}_i(t) \ge \frac{1}{2} + \frac{1}{2^{D_{\max}}}$}  \\ 
    \probc(\mu,\mu-g(\bar{N}_i(t))) = \theta> \theta' \ \ \text{if $\bar{N}_i(t) < \frac{1}{2} + \frac{1}{2^{D_{\max}}}$}  \\ 
\end{align}
Similar to the proof of Theorem \ref{th:NP_hard_same_gamma} we can obtain a utility of $(\theta-c) \cdot (T+1)$ if and only if we always pull from the first $k$ arms without violating their delay in the first $T$ rounds. Therefore, a \maxreward{} instance of Theorem \ref{th:blockingMAB_is_np_hard}
is a YES instance if and only if we can obtain a utility of $(\theta-c) \cdot (T+1)$ in our problem. 
\end{proof}

\input{approximation_proofs}

==> HOLDER_4.tex <==
Now we state the following theorem and give its proof 
\begin{restatable}{theorem}{NPhardsameshrinkage}\label{th:NP_hard_same_shrinkage}
Even when all of the arms have the same cost $c$ and the same shrinkage function $g(.)$ the problem of finding a pure optimal strategy for the human is NP-hard.  
\end{restatable}
\begin{proof}
We will follow a reduction similar to the previous of Theorem \ref{th:NP_hard_same_gamma}. The difference is that all arms will have the same shrinkage function $g(.)$ but the discount factor for the arms will be will different and set according to the delay value $D_i$. Moreover, the first $k$ arms will have a mean of $\mu=1$ and the last arm will have a mean of $\mu_{k+1}=0.6$. All arms will have a cost of $c=0.725$. The shrinkage function for all arms will be set to
\begin{align}
    g(n) = 0.6 - 0.3 n  
\end{align}
Since we will have $\max\limits_{i \in [k+1]} \gamma_i \leq \frac{1}{2}$ so that $N_i(t) \leq \frac{\gamma_i}{1-\gamma_i} \leq 1$, the above values immediately imply that we have $\maxgenmu{t} \ge \genmu{i}(t) \ge 0.4 > 0.3 \ge \genmu{k+1}(t) \ , \forall i \in \arms, t \in [T+1]$. Therefore, the AI will never pull arm $k+1$ since it always picks the arm with the maximum generative mean in each round. 

The following two claims follow from Claims \ref{cl:nbar_lower_bound} and \ref{cl:nbar_upper_bound}, they are simply restated for different values of $\gamma_i$. 
\begin{claim}\label{cl:lower_bound_discount}
If a pull violates the delay rule for an arm $i$ at round $t$, then we have:
\begin{align}
    N_i(t) \ge \gamma_i + \gamma_i^{D_i}
\end{align}
\end{claim}

\begin{claim}\label{cl:upper_bound_discount} 
If the delay rule for an arm $i$ is not violated then the discounted number of samples at any round $t$ is at most   
\begin{align}
    N_i(t) \leq \gamma_i \cdot \frac{1}{1-\gamma_i^{D_i}}
\end{align}
\end{claim}
We further have the following claim which is similar to Claim \ref{cl:half_special}.
\begin{claim}
$\forall \gamma_i \in (0,\frac{1}{2}]$ with $D_i \ge 2$ we have 
\begin{align}
    \gamma_i \cdot \frac{1}{1-\gamma_i^{D_i}} < \gamma_i + \gamma_i^{D_i}   \label{eq:discount_ineq}
\end{align}
\end{claim}
\begin{proof}
The proofs follows immediately by Lemma \ref{lemma:bound_f_gamma_D}. 
\end{proof}

For the last arm we set $\gamma_{k+1}=\frac{1}{2}$, but for the first $k$ arms with $D_i \ge 2$ we want to find values of $\gamma_i \in (0,\frac{1}{2}]$ such that violating the delay values results in the discounted number of samples $N_i(t)$ being at least $\gamma_i + \gamma_i^{D_i}$ with 
\begin{align}
     \gamma_i + \gamma_i^{D_i} = \frac{1}{2} \label{eq:viol_satisfy}
\end{align}
It is straightforward to see that for $D_i \ge 2$ there always exist values of $\gamma_i \in (0,\frac{1}{2}]$ such that \eqref{eq:viol_satisfy} is satisfied. To see that, note that the function $\gamma_i + \gamma_i^{D_i}$ is continuous and that $\gamma_i + \gamma_i^{D_i}\Big|_{\gamma=0}=0 < \frac{1}{2}$ and $\gamma_i + \gamma_i^{D_i}  \Big|_{\gamma=\frac{1}{2}} > \frac{1}{2}$. Note the following simple fact which will be helpful later
\begin{fact}
If $D_i \ge 2$ and $\gamma_i + \gamma_i^{D_i} = \frac{1}{2}$ then we must have $\gamma_i \ge 0.3$. 
\end{fact}
\begin{proof}
This follows since $\gamma_i + \gamma_i^{D_i}$ is an increasing function and $0.3 + 0.3^{D_i} \leq 0.3 + 0.3^{2} \leq 0.39 < \frac{1}{2}$. 
\end{proof}



Now, although the values of $\gamma_i$ that satisfy \eqref{eq:viol_satisfy} exist. It is not straightforward to find an exact closed form solution for them, so we will approximate them. Note that $\gamma_i + \gamma_i^{D_i}$ is increasing, therefore by doing binary search over the interval $[0.3,\frac{1}{2}]$ we can obtain an approximation. However, it is important to establish a bound on the desired approximation error. To do that we define the following function which equals the different between the lower bound when violating the delay rule and the upper bound when not violating it for a given value of $\gamma \in [0.3,\frac{1}{2}]$ and $D \ge 2$ 
\begin{align}
    h(\gamma,D) = \gamma + \gamma^D - \frac{\gamma}{1-\gamma^D}  
\end{align}
We now reach the following lemma
\begin{lemma}\label{lemma:min_seperation}
For $\gamma \in [0.3,\frac{1}{2}]$ and $D \ge 2$. Let $\delta =\frac{1}{3} \frac{1}{2^{\dmax}}$ then we have 
\begin{align}
     h(\gamma,D) \ge  \delta 
\end{align}
\end{lemma}
\begin{proof}
It is straightforward to show that $h(\gamma,D)$ is decreasing in both arguments for $\gamma \in [0.3,\frac{1}{2}]$ and $D \ge 2$. Therefore, it obtains the minimum value at $\gamma=0.5$ and $\dmax = \max\limits_{i \in \arms} D_i$ this lead to 
\begin{align}
    h(\gamma,D) & \ge h(0.5,\dmax) \\ 
                & = \frac{1}{2} + \frac{1}{2^\dmax} - \frac{\frac{1}{2}}{1-\frac{1}{2^\dmax}}\\
                & = \frac{1}{2^{\dmax}}  - \frac{1}{2} \cdot \frac{1}{2^{\dmax}-1} \\  
                & \ge  \frac{1}{2^{\dmax}} - \frac{2}{3} \frac{1}{2^{\dmax}} && \text{(since $\frac{1}{2} \cdot \frac{1}{2^{\dmax}-1} \leq \frac{2}{3} \frac{1}{2^{\dmax}}$ for $\dmax \ge 2$)} \\ 
                & = \frac{1}{3} \frac{1}{2^{\dmax}}
\end{align}
\end{proof}

Therefore, we will approximate $\gamma_i$ for the first $k$ arms so that \eqref{eq:viol_satisfy} holds within an error of at most $\frac{\delta}{4}$. We will now show that $O(\poly(k))$ iterations are sufficient for any arm $i$ with $D_i \ge 2$. %Note that $O(\log D_i)$ would be at most a polynomial number of iterations. 

\begin{lemma}
Let $R_0 = \frac{1}{2} -0.3=0.2$ and let $f_{D_i}(\gamma_i)=\gamma_i + \gamma_i^{D_i}$. Then for a given value of $D_i \ge 2$ after $\log_2 \big(\frac{4 (D_i+1) R_0}{\delta} \big)$ iterations of binary search for the function $f_{D_i}(\gamma_i)$ over $\gamma_i \in [0.3,0.5]$ if we obtain $\ghat_i$ then we have 
\begin{align}
    |f_{D_i}(\ghat_i) - \frac{1}{2}| \leq \frac{\delta}{4}
\end{align}
\end{lemma}
\begin{proof}
After $q$ many iterations of binary search over the interval $R_0=\frac{1}{2} -0.3=0.2$ the size of the search region will be $\frac{R_0}{2^q}$. Any returned solution $\ghat_i$ in this region will be at most at a distance of $\frac{R_0}{2^q}$ from the true solution $\gstari$ where $f_{D_i}(\gstari)=\frac{1}{2}$. Based on Lemma \ref{lemma:lipshitz_f} we will have 
\begin{align}
    |f_{D_i}(\ghat_i) -f_{D_i}(\gstari)| & \leq (D_i+1) \frac{R_0}{2^q} \\ 
                                          & = (D_i+1) \frac{R_0 \delta}{4 (D_i+1) R_0} \\
                                          & = \frac{\delta}{4}
\end{align}
\end{proof}
Note that since $\dmax = \poly(k)$, then it follows that $\log_2 \big(\frac{4 (D_i+1) R_0}{\delta} \big) = \log_2 \big(4 (D_i+1) R_0 \cdot 3 \cdot 2^{\dmax} \big) = O(\log \dmax) + O(\dmax) = \poly(k)$. 

We will denote with $\ghat_i$ the resulting approximated discounting factors. We note that using our approximation we can establish the following separation between the discounted number of pulls based on whether the delay rule was violated or not. Specifically, we have the following fact
\begin{fact}
For any arm $i \in \arms$ with $D_i \ge 2$ if at round $t-1$ the delay rule was violated then $N_i(t-1)\ge \frac{1}{2}- \frac{\delta}{4} > \frac{\ghat_i}{1-\ghat_i^{D_i}}$. On the other hand, if the delay rule was not violated at any round up to and including $t-1$ then we have $N_i(t-1)\leq \frac{\ghat_i}{1-\ghat_i^{D_i}} < \frac{1}{2} -\frac{\delta}{4}$. 
\end{fact}
\begin{proof}
Note that be Lemma \ref{lemma:min_seperation} we have for any $\ghat_i$ 
\begin{align}
    \ghat + \ghat^{D_i} \ge \frac{\ghat_i}{1-\ghat_i^{D_i}} + \delta 
\end{align}
Since our approximations for \eqref{eq:viol_satisfy} are up to an additive error of $\frac{\delta}{4}$, then it follows that if we violate the delay rule at round $t-1$ that we have 
\begin{align}
    N_i(t-1) = \ghat + \ghat^{D_i} \ge \frac{1}{2} - \frac{\delta}{4} 
\end{align}

Now if we do not violate the delay rule, then $N_i(t-1) \leq \frac{\ghat_i}{1-\ghat_i^{D_i}} < \ghat + \ghat^{D_i} \leq \frac{1}{2} - \frac{\delta}{4}$. 
\end{proof}


\SE{BEGIN BEGIN BEGIN} 




Let $g_u(\gamma,D) =  \gamma + \gamma^{D}$. Then it is clear that $g_u(.,D)$ is decreasing in $D$. Let $D_{\max} = \max_{i \in [K]} D_i$ then for the arms with delay $D_{\max}$ we set $\gamma_i=\gamma_{\max}=\frac{1}{2}$. For the other arms we will choose $\gamma_i \in (0,\frac{1}{2}]$ such that $\gamma_i + \gamma_i^{D_i} = \frac{1}{2} + \frac{1}{2^{D_{\max}}}$. This is possible since $g_u(\frac{1}{2},D_i) > g_u(\frac{1}{2},D_{\max}) = \frac{1}{2} + \frac{1}{2^{D_{\max}}}$ since $D_i < D_{\max}$ and since $\lim\limits_{\gamma_i \to 0^{+}}  g_u(\gamma_i,D_i) = 0 < g_u(\frac{1}{2},D_{\max})$. Since $g_u(\gamma,D_i)$ is continuous there must exist some value in $\gamma \in (0,\frac{1}{2}]$ such that $\gamma_i + \gamma_i^{D_i} = \frac{1}{2} + \frac{1}{2^{D_{\max}}}$. 

Setting $\gamma_i$ to such values would lead the discounted number of samples to be separated into two disjoint intervals based on whether the delay was violated as illustrated in Figure \ref{fig:diff_gamma} and proved in the following claim. 
\begin{claim}
If the arms $i \in \arms$ are pulled without violating the delay up to round $T$ then $\forall t\in [T+1]: \max_{i \in \arms} N_i(t) <  \frac{1}{2} + \frac{1}{2^{D_{\max}}}$ whereas if the delay is violated in any round up to and including $T$ then there exists at least one round $t \in [T+1]$ such that $\max_{i \in \arms} N_i(t) \ge \frac{1}{2} + \frac{1}{2^{D_{\max}}}$. 
\end{claim}
\begin{proof}
If we do not violate the delays then for any arm $i$ by Claim \ref{cl:upper_bound_discount} we have
\begin{align}
    N_i(t) & \leq \gamma_i \cdot \frac{1}{1-\gamma_i^{D_i}} \\ 
                 & < \gamma_i + \gamma_i^{D_i}  && \text{(by Lemma \ref{lemma:bound_f_gamma_D} and since $\gamma_i \in (0,\frac{1}{2}]$)} \\
                 & = \frac{1}{2} + \frac{1}{2^{D_{\max}}} && \text{(by construction of the values $\gamma_i$)}
\end{align}
The second part of the claim follows by construction and Claim \ref{cl:lower_bound_discount}.
\end{proof}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Pictures/diff_gamma.pdf}
    \caption{For any arm, once the delay is violated the discounted number of pulls will be at least $\frac{1}{2}+\frac{1}{2^{D_{\max}}}$.}
    \label{fig:diff_gamma}
\end{figure}

Now we set the values $\probc(.,.)$ for the first $k$ arms. 
\begin{align}
    \probc(\mu,\mu-g(N_i(t))) = \theta' \ \ \text{if $N_i(t) \ge \frac{1}{2} + \frac{1}{2^{D_{\max}}}$}  \\ 
    \probc(\mu,\mu-g(N_i(t))) = \theta> \theta' \ \ \text{if $N_i(t) < \frac{1}{2} + \frac{1}{2^{D_{\max}}}$}  \\ 
\end{align}
Similar to the proof of Theorem \ref{th:NP_hard_same_gamma} we can obtain a utility of $(\theta-c) \cdot (T+1)$ if and only if we always pull from the first $k$ arms without violating their delay in the first $T$ rounds. Therefore, a \maxreward{} instance of Theorem \ref{th:blockingMAB_is_np_hard}
is a YES instance if and only if we can obtain a utility of $(\theta-c) \cdot (T+1)$ in our problem. 
\end{proof}

==> analysis_1.tex <==
\section{Analysis}
\subsection{Some guarantees for the AI when it follows the max generative mean strategy} 
\SE{You can skip/skim this subsection if you had seen it before. }
We have two main results here. The first, shows that the AI maximizes its utility at a given round by selecting the maximum generative mean (Fact \ref{fact:mgm_maximizes_prob}) and that the AI will also be maximizing its total utility ($u_{\ai}(T)$) if the human follows an oblivious strategy where an oblivious strategy is independent of the user's pulls or AI actions (Theorem \ref{theorem:ai_best_resp_obv}). 

At a given round both the human and the AI will choose an arm with some probability. Let the probability vectors over the arms for round $t$ be $\theta_t$ and $\phi_t$ for the human and AI, respectively. Define the arm with the maximum generative mean as $\mgm(t)$, formally $\mgm(t)= \max\limits_{i \in \arms} \big( \mu_i - g_i(\pullsh{i}(t-1)) \big)$

We have the following fact: 
\begin{fact}\label{fact:mgm_maximizes_prob}
At round $t$ the AI maximizes the probability of being pulled by choosing the arm with the current highest generative mean $\mgm(t)$. 
\end{fact}
\begin{proof}
\begin{align}
    \Prob(a_t > b_t) & = \sum_{i,j \in [K]} \avec_t(j) \bvec_t(i) \probc(\Tilde{\mu}_i,\mu_j) \\ 
                   & = \sum_{i \in [K]} \bvec_t(i) \Big( \sum_{j \in [K]} \avec_t(j) \probc(\Tilde{\mu}_i,\mu_j) \Big) \\
                   & \leq \sum_{j \in [K]} \avec_t(j) \probc(\Tilde{\mu}_{\mgm(t)},\mu_j) && \text{(by the mean monotonicity property of $\probc$)}
\end{align}
\end{proof}

\begin{definition}[Oblivious human strategy] A strategy $S$ followed by the human is called oblivious if the actions selected by the human at any round $t$ are always independent of the actions taken by the AI or the user. Formally, denoting the human and AI histories up to round $t$ by $\histb(t)$ and $\hista(t)$ where the history of an agent up to round $t$ is the arm choices and realized rewards up to round $t$ of the agent. This history does not include the arms that were chosen by the user which we denote by $\histu(t)$. Then an oblivious strategy $S_{\text{obv}}$ has for any round $t$ that the choice of arm is independent of the AI's previous actions $\forall i \in \arms: \bvec_t(i;\histb(t-1),\hista(t-1),\histu(t-1))=\bvec_t(i;\histb(t-1))$. 
\end{definition}

\begin{observation} If the human's strategy is oblivious then it is independent of the AI's strategy.
\end{observation}

\begin{theorem}\label{theorem:ai_best_resp_obv}
If the human follows an oblivious strategy then the AI can maximize its utility by following the strategy of selecting $\mgm(t)$ in each round. 
\end{theorem}
\begin{proof}
The human follows an oblivious strategy $\sobv$. We will use a proof by induction, let $\smgm$ and $S'$ denote the $\mgm$ and some arbitrary strategy $S'$, respectively. 

\paragraph{Base Case:} $\uai(1;\sobv, \smgm) \ge \uai(1;\sobv,S')$ by Fact \ref{fact:mgm_maximizes_prob}. 

\paragraph{Inductive Step:} 
%By the hypothesis we have $\uai_{S^{\mgm}}(t-1) \ge \uai_{S}(t-1)$ and by Fact \ref{fact:mgm_maximizes_prob} we have $\probc(\mgm((t) > a_t) \ge  \probc(b^{S}_t > a_t)$. Therefore, $\uai_{S^{\mgm}}(t) \ge \uai_{S}(t)$.
Note that for any human and AI strategies $S_1$ and $S_2$ (respectively) the utility brakes down as 
\begin{align}
    \uai(t;S_1,S_2) = \uai(t-1;S_1,S_2) + \Prob(a(t) > b(t); S_1, S_2)  
\end{align}
Since the human's strategy is oblivious then it is independent of the AI's strategy and therefore the probability that the human will pull arm $i$ at round $t$ will be $\theta_t(i,\sobv)$ for both strategies $\smgm$ and $S'$. Therefore, it follows by Fact \ref{fact:mgm_maximizes_prob} that $\Prob(\mgm(t) > b(t); \smgm, \sobv) \ge \Prob(\mgm(t) > b(t); S, \sobv)$. Further, since $\uai(t-1;\smgm,\sobv) \ge \uai(t-1;S',\sobv)$ by the inductive hypothesis then $\uai(t;\smgm,\sobv) \ge \uai(t;S',\sobv)$.
\end{proof}


\paragraph{What if the human strategy is not oblivious?}
Here we show that the $\mgm$ strategy is not utility maximizing in the non-oblivious case by a counter example. Suppose $T=3$ and we have two arms such that $\mu_1 \gg \mu_2$. Further, the constant $c$ in $\frac{c}{\sqrt{1+\pullsh{i}(t-1)}}$ is very small so that $\Tilde{\mu}_i \approx \mu_i$ and therefore $\probc(\Tilde{\mu}_2,\mu_1) \leq \epsilon_1$, $\frac{1}{2} -\epsilon_2 \leq \probc(\Tilde{\mu}_1,\mu_1) \leq \frac{1}{2}$, $\probc(\Tilde{\mu}_1,\mu_2) \ge 1 -\epsilon_3$.

AI strategies are the following:
\begin{enumerate}
    \item $\mgm$: always pull arm 1. 
    \item $A_2$: pull arm 2 in the first round and then always pull arm 1. 
\end{enumerate}

The human's not oblivious strategy is a follows: pull arm 1 in the first round and keep pulling arm 1 if AI pulls arm 1 in the first round otherwise always pull arm 2
We have: 
\begin{align}
    & \uai(\mgm) \leq \frac{1}{2} T  = \frac{3}{2}  \\ 
    & \uai(A_2)  \ge 0 +  (1-\epsilon_3) \cdot 2 = 2(1-\epsilon_3) > \uai(\mgm)  \ \ \text{for sufficiently small $\epsilon_3$.}
\end{align}
But it is worth noting that this is not an equilibrium (human can deviate).

% \section{Two Regimes for the Horizon}
% We will assume that the arms are ordered by the mean, i.e. $\mu_1 \ge \mu_2 \dots \ge \mu_K$. For a given round $t$ set $\sumbvc_t = \sum_{i \in [K]} \bvec_t(i)$ which is the probability that the human will pull an arm (participate) at round $t$ then the human utility can be written as  
% \begin{align}
%     \uh(t) = \sum_{s=1}^t \E[\probc(\mu_{b_t},\mu_{a_t})  - \rho \sumbvc_t]  
% \end{align}
% Suppose the human follows a strategy of always pulling the arm with the highest mean $\mu_1$ then $\Tilde{\mu}_1(t)$ will keep increasing eventually we will have: 
% \begin{align}
%     \probc(\mu_1,\Tilde{\mu}_1(t)) - \rho < 0 
% \end{align}
% The human will therefore stop since the utility per round for participation becomes negative. In general, for a strategy $S$ we may define the first round where the human exists the system as: 
% \begin{align}
%     \tauexit(S) = \min t  \text{ s.t. } \probc(\mu_1,\Tilde{\mu}_{\mgm(t)}) - \rho < 0  \label{eq:tau_exit_incorrect_def}
% \end{align}
% By monotonicity of $\probc(.,.)$ it also follows that we will also have $\probc(\mu_i,\Tilde{\mu}_{\mgm(t)}) - \rho < 0 \ \forall i \in [K]$. 

% \paragraph{Refinement of the definition of $\tauexit$:} The above definition in \eqref{eq:tau_exit_incorrect_def} should be refined to exclude trivial strategies. Consider the case where $\mu_1 \gg \mu_2 \ge \mu_1 - c$ then if the human only pulls arm $2$ then we could always have $\mu_1 > \mu_{\mgm(t)}$. But this would lead the human to get negative utility. Therefore, $\tauexit$ is the optimal solution of the following optimization problem: 
% \begin{subequations} 
% \begin{equation}
%     \max\limits_{S} \min\limits_{t \ge 1} \ t
% \end{equation}
% \begin{equation}
%     \probc(\mu_1,\Tilde{\mu}_{\mgm(t)}) - \rho \leq 0
% \end{equation}
% \begin{equation}\label{eq:tau_exit_def}
%     \forall t'<t:  \ \probc(\mu_{b_{t'}},\Tilde{\mu}_{\mgm(t')})-\rho > 0 
% \end{equation}
% \end{subequations}
% The point behind the above is that if the horizon $T$ is large enough then there will be a round where the human would exit the system so that he would not lose utility. Accordingly, we can define two regimes for the horizon $T$. 

% \begin{definition}[Long Horizon] In the large horizon regime, $T$ is sufficiently large so that for any strategy followed by the human $S$ we have $\tauexit(S) \leq T$. 
% \end{definition}

% \begin{definition}[Short Horizon] In the small horizon regime, $T$ is sufficiently small so that there exists a strategy for the human $S$ so that $\tauexit(S) > T$. 
% \end{definition}

% \begin{observation}
% The definition of $\tauexit$ makes it independent of the strategy followed by the AI. Therefore to maximize it the human can follow an oblivious strategy. 
% \end{observation}

% \paragraph{Discounted Horizon Can Change This:} If we follow that discounted reward setting in $\frac{c}{\sqrt{1+\pullshdisc{i}(t-1)}}$ then even if the horizon has a very large value then there may exist a strategy where the human can always gain positive utility. 

% \newpage 


==> cycling.tex <==
\section{Does Cycling Work?}
Consider the case with $K=T$ arms with $\forall i: \mu_i=\mu, c_i=c, \gamma_i=\gamma$, however the growth functions are $g_1$ and $g_i=g \ \forall 2 \leq i \leq K$. Let $g_1$ be very slow so that even if the number of samples are $\frac{\gamma}{1-\gamma}$ we have $g_1(\frac{\gamma}{1-\gamma}) \leq \epsilon$. But for other growth functions we have $g_i(\gamma) \ge g \gg \epsilon$. 

\paragraph{Utility for a strategy that always pulls arm $1$:}
\begin{align}
    u(T) \ge  T \cdot \Big( \big[\probc(\mu,\maxgenmu{1}) - c \big]- \epsilon L_g L_{\probc} \Big)
\end{align}

\paragraph{Utility for a strategy that cycles among the arms:}
\begin{align}
    u(T) \leq  2 \cdot \Big( \probc(\mu,\maxgenmu{1}) - c\Big)  + T \cdot \Big( \big[\probc(\mu,\maxgenmu{1}) - c \big] - g L_g L_{\probc} \Big)
\end{align}

==> interpretation.tex <==
\section{Interpretation of the above result} 
We will extend our model to allow the user to not select either the human or AI and instead be idle. Specifically, we extend the probability to a 3 argument function $\probc(\mu_i,\mu_j,\muidle)$ where $\muidle$ is always constant and represents the user utility for not viewing the AI or human contributions. Note that $\probc$ maintains the same monotonicity properties. Define the user welfare through the horizon to be the following: 
\begin{align}
    w(T) = \sum_{t=1}^T \E[\mu_{I_t} \indic(\text{user select arm $I_t$})] \\
\end{align}

\subsection{Simple Analysis} 
Suppose that there was no AI in the system, then the the human can maximize utility by contributing the arm with the highest mean $\mu_1$, leading to: 
\begin{align}
    w^*(T) = \mu_1 T  
\end{align}

Now suppose that the AI enters the system and follows the max generative mean strategy, then to maximize utility the human follows algorithm \ref{alg:form_dag}. Suppose that we have $K$ arms with $\mu_1 > \mu_2=\mu_3=\dots=\mu_K$. Then as shown earlier the human would being by pulling all arms $\mu_i$ with $i \ge 2$ until the highest $p$ such that $\genmu{i}(p)\leq \genmu{1}(0)$. 

Let the constant $c > \Delta_2$, then we are looking for the maximum $\pmax$ such that $\mu_2 - \frac{c}{\sqrt{1+\pmax}} \leq \mu_1 -c$. By simple algebra we find that $\pmax \leq \big(\frac{c}{c-\Delta_2} \big)^2 -1$. Now if we upper bound the user welfare we would find: 
\begin{align}
    w(T) \leq (K-1) \pmax \mu_2 \probc(\mu_2, \genmu{1}(0)) + [T-(K-1)\pmax] \mu_1 \probc(\mu_1, \genmu{1}(0))
\end{align}

Suppose we are in a setting where $(K-1)\pmax = \beta T +o(T)$ where $\beta$ is a constant. Then the upper bound becomes: 
\begin{align}
    w(T) \leq \beta \mu_2 T + (1-\beta) T \mu_1 + o(T) 
\end{align}
If we calculate the welfare regret, then we would find that 
\begin{align}
    R(T) = w^*(T) - w(T) & \ge \beta \mu_1 T - \beta \mu_2 T  - o(T) \\ 
                         & \ge \beta \Delta_2 T - o(T) 
\end{align} 
if $\beta \Delta_2 = \Theta(1)$ then the user's regret is linear. 




\subsection{More Refined}
The problem with the above is that the model does not actually incentivize the human to contribute his best arm in the absence of the AI. We will generalize the probability choice to be $\probcg(\mu_i,\mu_j)$ where $\probcg$ allows the user to possibly not select either contribution and instead watch noting. Further, in the absence of two contributions (e.g., only human in the system) we will use $\probcg(\mu_i)$ to denote the probability that the user will select arm $i$ instead of selecting nothing. 
\begin{align}
    \probcg(\mu_i,\mu_j) = \text{prob of user selecting arm $i$ instead of $j$ or nothing}  \\
        \probcg(\mu_i) = \text{prob of user selecting arm $i$ instead of nothing}  
\end{align}
Higher values of $\gamma$ lead to higher probability for choosing nothing. Example of $\probcg$ is $\probcg(\mu_i, \mu_j, \muidle)= \frac{\mu_i}{\mu_i + \mu_j + \muidle}$. Another way to construct $\probcg$ is through $\probc$ where arm $\mu_i$ duels with $\muidle$, arm $\mu_j$ duels with $\muidle$ and the winner duels with the winner of $\mu_i$ and $\muidle$. This leads to $\probcg(\mu_i,\mu_j)= \probc(\mu_i,\muidle) \cdot \probc(\mu_j,\muidle) \cdot \probc(\mu_i,\mu_j) + \probc(\mu_i,\muidle) \cdot \probc(\muidle, \mu_j) \cdot \probc(\mu_i,\muidle)$. 

We assume that $\probcg$ satisfies the following properties:
\begin{align}
    \probcg(\mu_i,\mu_j,\muidle) & \ge \probcg(\mu_i,\mu'_j,\muidle) && \text{if $\mu'_j \ge \mu_j$} \\ 
    \probcg(\mu'_i,\mu_j,\muidle) & \ge \probcg(\mu_i,\mu_j,\muidle) && \text{if $\mu'_i \ge \mu_i$} \\ 
    \probcg(\mu_i,\mu_j,\muidle) & \leq \probcg(\mu_i,\muidle) \\
    \probcg(\mu'_i,\muidle) & \ge \probcg(\mu_i,\muidle) && \text{if $\mu'_i \ge \mu_i$} \\ 
    \probcg(\mu_i,\mu_i,\muidle) + \probcg(\mu_i,\mu_i,\muidle) = 2 \probcg(\mu_i,\mu_i,\muidle) & \leq (1+\delta) \probcg(\mu_i,\muidle)  \\ 
\end{align}



Note that the user gains a utility of zero when he selects nothing. Following this model, when there is no AI to increase the probability of being watched the human should contribute his best arm. Therefore, we have:
\begin{align}
    w^*(T) = \mu_1 \probcg(\mu_1) T  
\end{align}
For simplicity we will assume a setting where (1) $\gamma$ is small so that $\probcg() \approx \probc()$ (user almost always makes a selection instead of nothing). (2)$\probcg(\mu_i,\mu_j)\approx 1$ if $\mu_i \ge \mu_j$, user almost always selects the arm with the highest mean.(3) $\Delta_i$ is a constant. (4) $\mu_1 >\mu_i \ \forall i>1$. 

\begin{theorem}
$R(T)=\Omega(T)$ if and only if (A) $\exists i >1$ such that $\nexitopt{i}=\Omega(T)$ or (B) $(\mu_1-\genmuexit{1}) (T-\nexit{1})=\Omega(T)$. \SE{$\underbrace{(\mu_1-\genmuexit{1})}_{\text{AI performance gap}} \times \underbrace{(T-\nexit{1})}_{\text{rounds after the human exits}}$}
\end{theorem}
\begin{proof}
If (A) is true then the welfare can be upper bounded by
\begin{align}
    w(T) & \leq \mu_1 \probcg(\mu_1) (T-\nexitopt{i}) + \mu_i \probcg(\mu_i) \nexitopt{i} \\ 
         & \leq \mu_1 \probcg(\mu_1) (T-\nexitopt{i}) + \mu_i \probcg(\mu_1) \nexitopt{i} \\ 
         & \approx \mu_1 (T-\nexitopt{i}) + \mu_i \nexitopt{i}
\end{align}
This leads to
\begin{align}
    R(T) & = w^*(T) - w(T) \\ 
         & \ge \mu_1 \probcg(\mu_1) T - \big(\mu_1 \probcg(\mu_1) (T-\nexitopt{i}) + \mu_i \probcg(\mu_1) \nexitopt{i}\big) \\
         & = \probcg(\mu_1) \Delta_i \nexitopt{i} \\ 
         & = \probcg(\mu_1) \Delta_i T - o(T) \\
         & \approx \Delta_i T - o(T)
\end{align}
Now if (B) is true (we assume that (A) is false as otherwise we have $R(T)=\Omega(T)$) then the upper bound is
\begin{align}
    w(T) = \mu_1 \probcg(\mu_1) \nexitopt{1} + \genmuexit{1} \probcg(\mu_1) (T-\nexitopt{1}) + o(T)
\end{align}
This leads to
\begin{align}
    R(T) & \ge \mu_1 \probcg(\mu_1) T   - (\mu_1 \probcg(\mu_1) \nexitopt{1} + \genmuexit{1} \probcg(\mu_1) (T-\nexitopt{1}) ) \\ 
         & = (\mu_1 - \genmuexit{1}) \probcg(\mu_1) (T - \nexitopt{1}) \\
         & \approx (\mu_1 - \genmuexit{1}) (T - \nexitopt{1}) \\ 
         & = \Omega(T)
\end{align}
Suppose both (A) and (B) are false, then we the lower bound is 
\begin{align}
w(T) & \ge \mu_1 \probcg(\mu_1) \nexitopt{1} + \genmuexit{1} \probcg(\genmuexit{1}) (T-\nexitopt{1}) + o(T)  \\ 
\end{align}
This leads to
\begin{align}
    R(T) & \leq \mu_1 \probcg(\mu_1) T - \big( \mu_1 \probcg(\mu_1) \nexitopt{1} + \genmuexit{1} \probcg(\genmuexit{1}) (T-\nexitopt{1}) - o(T)\big) \\ 
         & \approx (\mu_1 - \genmuexit{1}) (T - \nexitopt{1}) \\ 
         & = o(T)
\end{align}
\end{proof}





\subsection{Refined and Simple}
Define the welfare regret to be:
\begin{align}
    R_w(T) = \mu_1 T - \sum_{t=1}^T \E[\mu_{I_t} \indic(\text{user select arm $I_t$})] 
\end{align}
Suppose we have (1) $\probc(.,.)$ such that the arm with the largest mean is chosen with probability 1 and (2) The means $\mu_i$ are constant. This implies that the $\Delta_i$'s are constant. 
\begin{theorem}
$R(T)=\Omega(T)$ if and only if (A) $\exists i >1$ such that $\nexitopt{i}=\Omega(T)$ or (B) $(\mu_1-\genmuexit{1}) (T-\nexit{1})=\Omega(T)$. \SE{$\underbrace{(\mu_1-\genmuexit{1})}_{\text{AI performance gap}} \times \underbrace{(T-\nexit{1})}_{\text{rounds after the human exits}}$}
\end{theorem}
\begin{proof}
Suppose (A) is true,  let $\Tilde{\mu}_{s}$ be the highest generative mean during the rounds where the human pulls arm $i$
\begin{align}
    w(T) & \leq \mu_1  (T-\nexitopt{i}) + \mu_i \probc(\mu_i,\Tilde{\mu}_{s}) \nexitopt{i} \\ 
         & \leq \mu_1  (T-\nexitopt{i}) + \mu_i \nexitopt{i} && \text{(since $\mu_i \ge \muexit{i} > \Tilde{\mu}_{s}$, thus $\probc(\mu_i,\Tilde{\mu}_{s})=1$)}
\end{align}
This leads to
\begin{align}
    R(T) & = w^*(T) - w(T) \\ 
         & \ge \mu_1 T - \big(\mu_1  (T-\nexitopt{i}) + \mu_i \nexitopt{i}\big) \\
         & =  \Delta_i \nexitopt{i} \\ 
         & =  \Delta_i T - o(T) 
\end{align}
Now if (B) is true (we assume that (A) is false as otherwise we have $R(T)=\Omega(T)$) then the upper bound is
\begin{align}
    w(T) = \mu_1 \nexitopt{1} + \genmuexit{1} (T-\nexitopt{1}) + o(T)
\end{align}
This leads to
\begin{align}
    R(T) & \ge \mu_1  T   - (\mu_1  \nexitopt{1} + \genmuexit{1}  (T-\nexitopt{1}) ) - o(T)\\ 
         & = (\mu_1 - \genmuexit{1})  (T - \nexitopt{1})  - o(T) \\
         & = \Omega(T) 
\end{align}
Suppose both (A) and (B) are false, then we the lower bound is 
\begin{align}
w(T) & \ge \mu_1 \nexitopt{1} + \genmuexit{1} (T-\nexitopt{1}) + o(T)  \\ 
\end{align}
This leads to
\begin{align}
    R(T) & \leq \mu_1  T - \big( \mu_1  \nexitopt{1} + \genmuexit{1}  (T-\nexitopt{1}) + o(T)\big) \\ 
         & = (\mu_1 - \genmuexit{1}) (T - \nexitopt{1}) - o(T) \\ 
         & \leq o(T)
\end{align}
\end{proof}

==> introduction_May_21_10_20pm.tex <==
\section{Introduction}
The emergence of Generative Artificial Intelligence (GenAI) has ushered in a trans-formative era across numerous practical domains, including text~\cite{chatgpt}, image~\cite{imagen}, and video generation~\cite{ho2022imagen, bartal2024lumiere, sora}. As AI-generated content proliferates on online platforms, ranging from video-sharing websites, e.g., YouTube and TikTok, to news outlets, the implications for human content creators are profound. %This paper examines the evolving dynamics between human and AI creators in the online platforms.

The rise of GenAI presents both challenges and opportunities for human content creators. While GenAI poses a competitive threat due to its capacity for rapid and cost-effective content generation, it also relies on human-created data for training and refinement. This interdependence creates a strategic interplay where human creators may adapt their content strategies to differentiate themselves from AI-generated outputs. A key concern surrounding GenAI is its potential to displace human creators due to its lower production costs and its capability to generate useful content as well as human creators. In the paper, we uncover that this threat can be real when the quality of AI-generated content is not discounted by the time of content generated by human creators and human creators will eventually \emph{exit} the platform. This model, termed as \emph{Long-horizon} setting in the paper, captures the practical scenarios that content information is not very timely, e.g., scientific knowledge sharing and professional skills training.

However, the imperative for timely and accurate content in online platforms necessitates a continuous influx of human-generated material to serve as training data for AI models, for example, financial information sharing and recent news comments. This reliance on human input suggests a cyclical relationship where the absence of human content could degrade the quality of AI-generated outputs, leading to user dissatisfaction and a renewed demand for human creativity. In this scenario, human creators may experience a resurgence in value as their content garners increased attention and engagement from users, which creates an intrinsic difficulty to analyze the dynamics between human and GenAI competition. To capture this scenario, we discount the human samples by the time when they are generated (the older the samples the more discounted) when we model the reward of GenAI.



\subsection{Our Contributions}
Our main contributions are threefold: 
\textbf{(1)} In Section \ref{sec:model}, we introduce the first model for dynamic competition between a human agent and a GenAI agent for content creation across different topics in an online platform. Our model introduces key elements that capture the advantages and disadvantages of both the human and AI agents. In addition, our model enables us to associate with each topic a measure of information ``freshness'' by discounting the samples available for a topic according to how recently they were generated, e.g., samples for topics such as news are more discounted than samples for topics such as history. Further, we introduce the myopic AI strategy and prove some of its optimality results. 

\SE{say consider the time-sensetive domain where topics need samples to be recent ``fresh'' and therefore have a non-trvial discounting samples}
\textbf{(2)} In Section \ref{sec:discounted} we study the setting where the samples for all topics are discounted by some non-trivial factor. Interestingly, we prove that it is NP-hard for the human to optimize his utility in this setting. We then introduce a simple approximation algorithm that alternates between running an optimization algorithm and pausing and show that it essentially has an approximation ratio of $\frac{1}{2}$. Finally, we prove that it is necessary for any algorithm in this setting to pause for a portion of the horizon as otherwise it may obtain a vacous approximation of the optimal utility.  

\SE{we consider domains where information for topics don't loose value with time.  interestingly we show it's solvable in polynomial time unlike the the previous}
\textbf{(3)} In Section \ref{sec:long_horizon}, we consider the long horizon setting with undiscounted samples. In this setting, it is impossible for the human to keep generating content and still gain non-negative utility and thus the human has to ``exit'' the platform at some round. However, the optimal utility maximizing strategy for the human is non-trivial to obtain and we show how simple baselines run in exponential time. We resolve this by identifying a collection of simplifying properties which an optimal strategy can satisfy to obtain a polynomial time algorithm. 


Due to space limits all proofs are moved to the Appendix.  

\hf{Emphasize contributions use the paper title --- it means we are at the shoes of content creator and it means a prescriptive approach of algorithm design, rather than a descriptive approach of equilibrium characterization. 

Our model is simple and basic. It captures certain essence of the dynamic competition but admittedly does not capture the whole landscape of the competition. We can see various ways to extend our basic model formulation which cannot be all covered in a single work (see our discussions in Conclusion section), but we believe our algorithmic results does offer useful insights for future studies of richer and concrete problem settings. }

==> misc.tex <==
\section{Suggestions for Model Modifications and Generalizations}
Here are some notes and modifications to the model we had discussed:
\begin{enumerate}
    \item \textbf{Discounted with arm (topic) specific discounting factor:} The generative mean for an arm (topic) $i$ uses a discounted value of the past pulls which at round $t$ equals 
    \begin{align}
        \pullshdisc{i}(t) = \sum_{s=1}^t \gamma^{t-s}_i \indic[b_s=i]  \ \ \text{where $\gamma_i \in (0,1]$}
        \genmu{i}(t) = \mu_i - \frac{c}{\sqrt{1+\pullshdisc{i}(t)}}        
    \end{align}
    We expect topics with large discount factors (such as news) to be difficult for the AI to compete in. Further, if $\gamma_i=1$ then we recover the original setting.  
    \item \textbf{Window Model:} (1) Using something similar to discounting, i.e. count the pulls only within the last window. (2) User can select any contribution within the window not just the ones at round $t$. 
    \item \textbf{Linear and Contextual Bandits:} Each user arriving at round $t$ has a context associated with him. The human and AI output a vector and the reward is the dot product with the user's vector. 
    \item \textbf{User may choose no arm (neither human nor AI)}. 
    \item \textbf{Possibility of Collusion between the human and the AI?} Can the human and AI have an equilibrium with a collusive strategy where the users on the platform possibly sees small rewards? 
\end{enumerate}

==> new_alg.tex <==
\subsection{New Algorithm}


The difficulty in the case of the discounting factor as opposed to the window case is that the number of pulls never go back to zero and therefore this makes things more complicated. Define $\gmax$ to be 
\begin{align}
    \gmax = \max\limits_{i \in [K]} \gamma_i
\end{align}

We handle this setting under the following condition
\paragraph{Condition:} $\forall i \in [K]: \gamma_i \leq \gmax <1$.   
Note that the problem remains hard even if there is an upper bound on all discounting factors so that $\gamma_i \leq \gmax<1$.

Let $s$ be the minimum positive possible utility possible \emph{per round}. For a given constant value $\epsilon >0$ we look for $\tauwindow$ such that the following is true: 
\begin{align}
    \frac{\gmax}{1-\gmax} \cdot \gmax^{\tauwindow} \leq \frac{1-\gmax}{L_g L_{\probc}} \cdot s \label{eq:tauwindow_construc_min_util}
\end{align}
We will use $\ntau$ to denote the left hand side of the above inequality, i.e.
\begin{align}
    \ntau = \frac{\gmax}{1-\gmax} \cdot \gmax^{\tauwindow} \label{eq:neps_def}
\end{align} 
Note that the left hand side approaches $0$ as $\tauwindow$ approaches $\infty$ and therefore we can always satisfy the above inequality by making $\tauwindow$ sufficiently large. If $s = \Omega(1)$ then the value of $\tauwindow$ needed to satisfy the above inequality is constant. 
\SE{since $\epsilon, \gmax, L_g, L_{\probc}$ are treated as constants $\tauwindow$ would still be a constant, but it seems reasonable to establish upper bounds.}

Further, we have that all growth functions are Lipschitz. Specifically, 
\begin{condition}
For all $i \in [K]$ we have:
\begin{align}
    |g_i(n_1) - g_i(n_2)| \leq L_g \cdot |n_1-n_2|
\end{align}
\end{condition}


Similarly the choice probability also has a Lipschitz property: 
\begin{condition}
\begin{align}
    |\probc(\mu,\mu_1) - \probc(\mu,\mu_2)| \leq L_{\probc} \cdot |\mu_1-\mu_2|
\end{align}
\end{condition}



Similar to the window case we can optimize over a small number of rounds $\tauwindow$ and this can be done in polynomial time if $\tauwindow$ is a constant\footnote{Note however that unlike the window case we will use the discounting factor to find the values of the generative means.}. Further, through an identical proof we can obtain the same lemma that shows that myopic optimization leads to the highest utility over $\tauwindow$ rounds
\begin{lemma}\label{lemma:myopic_opt_taudiscount}
Let $S^*$ be a pure optimal strategy for the human, then for any subset of $\tauwindow$ consecutive rounds starting from some value $t$ and ending at $t+(\tauwindow-1)$ we have 
\begin{align}
    \myopicopttau \ge u_{S^*}(t: t+ \tauwindow -1)
\end{align}

\end{lemma}
We follow the same algorithm as before, we will write it down again
\begin{algorithm}[h!] 
    \caption{\textsc{Myopically-Optimize-then-Halt}}\label{alg:myopic_then_halt_discount}
    \begin{algorithmic}[1]
    \STATE Set $\tauwindow = W_{\max}$.
    \STATE Solve utility maximization up to round $\tauwindow$ and call this strategy $S_{\myopic}(\tauwindow)$.
    \WHILE{$t \leq T$} 
    \STATE Alternate between following strategy $S_{\myopic}(\tauwindow)$ and halting for $\tauwindow$  many rounds. 
    \ENDWHILE
    \end{algorithmic}
\end{algorithm}

We now have the following theorem which establishes the approximation ratio of \textsc{Myopically-Optimize-then-Halt}. 
\begin{theorem}
\textsc{Myopically-Optimize-then-Halt} (algorithm block \ref{alg:myopic_then_halt_discount}) has an asymptotic approximation ratio of $\frac{1-\frac{1}{\tauwindow}}{2}$. 
\end{theorem}
\begin{proof}
Let $i_0$ be the arm that has the maximum number of discounted pulls at the end of in $S_{\myopic}(\tauwindow)$ and denote that number of pulls by $\bn_0$. Unlike the window case we cannot halt so that the number of pulls for all arms becomes zero. However, will will show that at the beginning of any epoch the number of pulls for any arm will be small. Specifically, we have
\begin{claim}
At the beginning of any epoch at round $t$ we have $\forall i \in [K]$ we have $\bn_i(t) \leq \ntau$. 
\end{claim}
\begin{proof}
Arms only receive pulls when $S_{\myopic}(\tauwindow)$ is active. It follows that after the end of $S_{\myopic}(\tauwindow)$ in the first epoch we have
\begin{align}
    \bn_0 \leq \sum_{r=1}^{\tauwindow} \gamma^r_{\max} = \frac{\gmax}{1-\gmax} \cdot (1-\gmax^{\tauwindow}) \leq \frac{\gmax}{1-\gmax} \cdot (1-\gmax^{2\tauwindow})
\end{align}
At the beginning of the $m^{th}$ epoch we would have an upper bound for the discounted number of pulls of (see Figure \ref{fig:discounted_pulls_bound})
\begin{align}
    \bn_0 \cdot \big(\gamma^{\tauwindow}_{\max} + \gamma^{3 \tauwindow}_{\max} + \gamma^{5 \tauwindow}_{\max} + \dots \big) & = \bn_0 \sum_{\ell=0}^{\infty} \gamma^{\tauwindow (2\ell+1)} \\
    & = \bn_0 \frac{\gamma^{\tauwindow}}{1-\gamma^{2\tauwindow}} \\
    & \leq \frac{\gmax}{1-\gmax} \cdot \gamma^{\tauwindow} \\
    & \leq \ntau && \text{(Based on \eqref{eq:tauwindow_construc} and \eqref{eq:neps_def})}
    \end{align}
\end{proof}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{Pictures/discounted_pulls_bound.pdf}
    \caption{}
    \label{fig:discounted_pulls_bound}
\end{figure}

Now we establish that $S_{\myopic}(\tauwindow)$ is approximately optimal if $\forall i \in [K]$ we have $\bn_i(t) \leq \ntau$.
\begin{claim}
Suppose we run the $S_{\myopic}(\tauwindow)$ starting from a state where the number of pulls for all arms is at most $\ntau$ then the utility we obtain is at least $(1-\epsilon) \cdot \myopicopttau$.     
\end{claim}
\begin{proof}
We will add a prime $'$ to denote a quantity when the number of pulls is starting from at most $\epsilon$, if it starts from $0$ then we omit the prime $'$. If we follow strategy $S_{\myopic}(\tauwindow)$ then at any round $r$ in the start of the epoch we would have $\bn'_i(r) \leq \bn_i(r) + \ntau \gamma^{r-1}$. It follows by the Lipshitz property of $g_i(.)$ and the fact that it is a decreasing function that $g_i(\bn'_i(r)) \ge g_i(\bn_i(r)) - L_g \ntau \gamma^{r-1}$. Therefore, the maximum generative mean increases by at most $L_g \ntau \gamma^{r-1}$, i.e. $\maxgenmu{r}' \leq \maxgenmu{r} + L_g \ntau \gamma^{r-1}$.  Further, it follows by the Lipshitz property of $\probc$ that in the first half of the epoch the utility is : 
\begin{align}
    \sum_{r=1}^{\tauwindow} \probc(\mu_{b_r},\maxgenmu{r}') - c_{b_r} & \ge \sum_{r=1}^{\tauwindow} \probc(\mu_{b_r},\maxgenmu{r} + L_g \ntau \gamma^{r-1}) - c_{b_r} \\
    & \ge \Big[\sum_{r=1}^{\tauwindow} \probc(\mu_{b_r},\maxgenmu{r} ) - c_{b_r}\Big] - \Big[ \sum_{r=1}^{\tauwindow}  L_g L_{\probc} \ntau \gamma^{r-1} \Big] \\
    & \ge \Big[\sum_{r=1}^{\tauwindow} \probc(\mu_{b_r},\maxgenmu{r} ) - c_{b_r}\Big] -  L_g L_{\probc} \ntau \frac{1}{1-\gmax} \\ 
    & \ge  \myopicopttau - s  && \text{(Based on \eqref{eq:tauwindow_construc} and \eqref{eq:neps_def})} \\
    & \ge  \myopicopttau - \frac{1}{\tauwindow} \myopicopttau  && \text{(since $\myopicopttau \ge s \cdot \tauwindow$)} \\
    & = (1-\frac{1}{\tauwindow}) \myopicopttau 
\end{align}
\end{proof}
The proof follows from the above. 
\end{proof}


\begin{corollary}
Using \textsc{Myopically-Optimize-then-Halt} we can obtain an approximation ratio of at least $\frac{1-\epsilon}{2}$ where $\epsilon$ is a constant. 
\end{corollary}
\begin{proof}
Simply set $\tauwindow$ so that $\frac{1}{\tau} \leq \epsilon$.
\end{proof}


\paragraph{Notes:} (1) We are assuming that $T$ is sufficiently large (asymptotic) so we can always find a suitable $\tauwindow$. (2) If $s=\Omega(1)$ then $\tauwindow = O(1)$, if $s=\Omega(T)$ then $\tauwindow=o(1)$. 


% \subsection{Impossibility of Approximation Under Arbitrarily Small $s$}
% \begin{theorem}
% For arbitrary $s$ no polynomial time $\alpha$-approximation algorithm with $\alpha >0$ can be obtained unless $P=NP$.  
% \end{theorem}
% \begin{proof}
% Follow the same reduction from blocking bandits. Set $\theta' -c < 0$, $\nu_0 < 0$ and $\theta -c = s$. Then the optimal algorithm would have a utility of $s  T$ whereas a sub-optimal algorithm would have at most $s  (T-1)$. Therefore, the approximation ratio is 
% \begin{align}
%     \frac{s (T-1)}{sT} = 
% \end{align}
% \end{proof}


==> notes.tex <==
\section{Probability of being pulled is not necessarily maximized by selecting the arm with the highest expected value} 
Here we show through a counter example that the selecting the arm with the maximum expected reward does not necessarily lead to a higher probability of being pulled. 

First, for ease of notation let $r_1$ and $r_2$ be the rewards of the human and AI respectively. Then the selection probability is $\frac{e^{\beta r_1}}{e^{\beta r_1}+e^{\beta r_2}}$ and $\frac{e^{\beta r_2}}{e^{\beta r_1}+e^{\beta r_2}}$ for the human  and AI, respectively. Note that $\beta \in [0,\infty)$ and when $\beta=0$ the probability is a $\frac{1}{2}$ for each whereas for $\beta \xrightarrow[]{}\infty$ the arm with highest reward is sampled with probability $1$.

\subsection{Counter Example} 
Suppose we have two arms $a_1$ and $a_2$. For $a_1$ the distribution is deterministic with $\mu_1=\frac{1}{2}$, $a_2$ has a Bernoulli distribution and takes the value of $1$ with probability $0.1$ (this implies that $\mu_2=0.1$).  

Since when the AI pulls the arm the reward is subtracted from we assume that the subtractions are $0.25$ and $0.05$ for arms $a_1$ and $a_2$, respectively. This implies that $0.25 = \mu_1 - f(n_1) > \mu_2 - f(n_2)=0.05$. 

Let's assume that the human will pull arm $a_1$ and calculate $p(a_1)$ and $p(a_2)$ which are the probability (utility) for the AI agent to be pulled for the next round if it pulls arm $a_1$ or $a_2$, respectively. If we assume that $\beta \xrightarrow[]{}\infty$ then we clearly have: 
\begin{align}
    p(a_1) = 0  \\ 
    p(a_2) = 0.05   
\end{align}
from the above $p(a_2) > p(a_1)$ although  $\mu_1 - f(n_1) > \mu_2 - f(n_2)$. This example can also be produced with finite $\beta$ that is sufficiently large. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\linewidth]{Pictures/counter_example.jpeg}
    \caption{Counter Example.}
    \label{fig:enter-label}
\end{figure}
\subsection{Special Case where the Probability is Maximized Using Maximum Expected Reward Value: Bernoulli Distribution} 
At a given round $t$ let $r_p$ and $r_h$ be the random variables that denote the rewards from the AI and human. Then for the AI, we have: 
\begin{align}
    \Pr(\text{at round $t$ the AI is chosen by the user}) = \E_{r_p,r_h}[\frac{e^{\beta r_p}}{e^{\beta r_p}+e^{\beta r_h}}]
\end{align}

Let $\theta^p_i$ and $\theta^h_i$ denote the probability that arm $i$ will be pulled by the AI and human, respectively. Since the AI and human decisions are made simultaneously in a given round, then we have: 
\begin{align}
    \E_{r_p,r_h}[\frac{e^{\beta r_p}}{e^{\beta r_p}+e^{\beta r_h}}] = \sum_{i,j \in \arms} \theta^p_i \theta^h_j  \E_{r_i,r_j}[\frac{e^{\beta r_i}}{e^{\beta r_i}+e^{\beta r_j}}]
\end{align}
If we let the reward distributions be Bernoulli, then we have the following: 
\begin{align}
    \E_{r_i,r_j}[\frac{e^{\beta r_i}}{e^{\beta r_i}+e^{\beta r_j}}] & = 
    (1-p_i) (1-p_j) \frac{e^{\frac{-c\beta}{\sqrt{n_i}}}}{e^{\frac{-c\beta}{\sqrt{n_i}}}+1} \\ 
    & + (1-p_i) p_j \frac{e^{\frac{-c\beta}{\sqrt{n_i}}}}{e^{\frac{-c\beta}{\sqrt{n_i}}}+e^{\beta}} \\ 
    & + p_i (1-p_j) \frac{e^{\beta \frac{(1-c)}{\sqrt{n_i}}}}{e^{\beta \frac{(1-c)}{\sqrt{n_i}}}+1} \\
    & + p_i p_j  \frac{e^{\beta \frac{(1-c)}{\sqrt{n_i}}}}{e^{\beta \frac{(1-c)}{\sqrt{n_i}}}+e^{\beta}} 
\end{align}
By collecting the terms we see that the expectation is strictly increasing in $p_i$ (note that $\E[r_i]=p_i$ since it is a Bernoulli distribution). Therefore, the AI's dominate strategy is to pick the arm with maximum expected value. 

\SE{Note: Can we have prove this result over a more general class, possibly having an upper bound on $\beta$. }




%\section{Solving the case where the means are known} 



==> old_max_utility.tex <==
\section{How does the human maximize the exit time?}

We make the following notes: 
\begin{enumerate}
    \item We are in the \emph{long horizon} setting. 
    \item $\mu_1 > \mu_2 > \dots > \mu_K$. 
    \item \textbf{Exit mean $\muexit{i}$:} For an arm $i$ we define $\muexit{i}$ as the smallest value such that for arm $i$ we have $\probc(\mu_i,\muexit{i}) -\rho <0$. It follows if $\Tilde{\mu}_i \ge \muexit{i}$ then $\probc(\mu_i,\Tilde{\mu}_i) -\rho <0$. Note that $\muexit{i}$ depends on the choice probability function $\probc$ and the mean of the arm $\mu_i$. 
    \item \textbf{Exit pulls $\nexit{i}$:} For an arm $i$ we define $\nexit{i}$ to be the smallest number $n$ such that $\mu_i - \frac{c}{\sqrt{1+n}} \ge \muexit{i}$. This implies that arm $i$ is pulled $\nexit{i}$ times by the human then $\genmu{i} \ge \muexit{i}$. 
\end{enumerate}

\begin{assumption}\label{assump:seperated_means}
For convenience, the means of the arms are sufficiently separated: for any $i$ and $j$ with $\mu_i <\mu_j$ then $\mu_i-\frac{c}{\sqrt{1+\nexit{i}}} < \muexit{j}$. This condition implies that if one more pull at round $t$ makes $\mgm(t)=i$ then we still have $\mu_{\mgm(t)} < \muexit{j}$.
\end{assumption}
Here we want to maximize the amount of time until the human exits the system while gaining positive utility in each round. Algorithm  \ref{alg:maximize_exit_large_gap} does that by essentially slowing down the increase in the generative means $\Tilde{\mu}_i$ starting from the smallest. Note that we define the set $A_{\mgm}(0)$ as follows:
\begin{align}
    \agmgm(t) = \{i \in \arms | \muexit{i} > \Tilde{\mu}_{\mgm(t)}\}
\end{align}
This implies that only pulling arms in $\agmgm(t)$  can give non-negative utility. See the attached Figure.



\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Pictures/n_exit_diagram.jpg}
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{Pictures/A_mgm_0.jpg}
    \caption{}
    \label{fig:enter-label}
\end{figure}

\begin{algorithm}[h!]
Find $\agmgm(0)$. Let $\barK = |\agmgm(0)|$.   \\ 
Set $p = \barK$. 
From round $t=1$ to $T$:  \\ 
    \ \ Pull arm $a_{p}$. \\ 
    \ \ If arm $p$ has been pulled $\nexit{p}$ many times then set $p=p-1$.\\ 
    \ \ Exit if $p=0$. 
\caption{\textsc{Maximize Exit Time: Gap Between Means}}\label{alg:maximize_exit_large_gap}
\end{algorithm}


% \begin{algorithm}[h!]
% Find $A_{\mgm}(0)$.  \\ 
% Group the arms: $\forall i,j \in \arms$ if $\mu_j = \mu_i$, then $i$ and $j$ are grouped. \\
% Order the Groups Based on the smallest mean within the group: $G_1, G_2, \dots, G_\ell$. \\ 
% From round $t=1$ to $T$:  \\ 
%     \ \ Alternate is pulling arms from the smallest group. \\ 
%     \ \ if $\Tilde{\mu}_{\mgm(t)} \ge \mu_i -\delta$ then deactivate $i$ and its group and never pull it again. 
% \caption{\textsc{Maximize Exit Time}}\label{alg:maximize_exit}
% \end{algorithm}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Pictures/ex_1.jpeg}
    \caption{Different Means.}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Pictures/ex_2.jpeg}
    \caption{Same Mean.}
    \label{fig:enter-label}
\end{figure}

\begin{theorem}\label{th:max_exit_time_large_gap}
Algorithm \ref{alg:maximize_exit_large_gap} maximizes the exit time under Assumption \ref{assump:seperated_means}.
\end{theorem}
\begin{proof}
\begin{fact}\label{fact:max_bound}
For any strategy (possibly randomized) followed by the human in any realization we have $\tauexit \leq \sum_{i \in \agmgm(0)} \nexit{i}$.  
\end{fact}
\begin{proof}
In any pull the human can only choose from the set $\agmgm(0)$ to gain non-negative. Since any arm $i \in \agmgm(0)$ can be pulled at most $\nexit{i}$ before the utility becomes negative the above follows.  
\end{proof}
\begin{fact}\label{fact:genmu_below_exit}
For any two arms $i,i'$ with $i>i'$ in the first round where $\genmu{i'} \ge \muexit{i'}$ we have $\genmu{i'} < \muexit{i}$. 
\end{fact}
\begin{proof}\label{fact:start_over}
This follows by the assumption made in Assumption \ref{assump:seperated_means} above. 
\end{proof}
\begin{fact}
At any round $t$ the algorithm only pulls from the set $\agmgm(t)$ and therefore the per round utility is always non-negative. 
\end{fact}
\begin{proof}
This follows by definition of $\agmgm(t)$ from the previous fact (Fact \ref{fact:genmu_below_exit}).
\end{proof}

\begin{fact}
Each arm is pulled $\nexit{i}$ many times. 
\end{fact}
\begin{proof}
After the first round $t$ where an arm $i \in [\barK]$ with $i>1$ that has been pulled $\nexit{i}$ many times we have for $\genmu{i-1(t)}=\mu_i - \frac{c}{\sqrt{1+\pullsh{i}(t-1)}}$ with $\pullsh{i}(t-1)=0$. Therefore by Fact \ref{fact:start_over} arm $i-1$ can be pulled $\nexit{i-1}$ many times.  
\end{proof}
From the above it follows that the total number of rounds is $\sum_{i \in \agmgm(0)} \nexit{i}$ and by Fact \ref{fact:max_bound} is it optimal. 
\end{proof}
\SE{add figure which explains the situation} \\ 
\SE{add fig for the special case of the algorithm}

\subsection{What if more than one arm has the same mean?} 
Here we assume that the arms either have the same mean or that they have a large separation so we have the following assumption.

\begin{assumption}\label{assump:seperated_means_or_nonun}
For convenience, the means of the arms are either the same mean ($\mu_i=\mu_j$) or are sufficiently separated: for any $i$ and $j$ with $\mu_i <\mu_j$ then $\mu_i-\frac{c}{\sqrt{1+\nexit{i}}} < \muexit{j}$. This condition implies that if one more pull at round $t$ makes $\mgm(t)=i$ then we still have $\mu_{\mgm(t)} < \muexit{j}$.
\end{assumption}

\begin{algorithm}[h!]
Find $\agmgm(0)$.  \\ 
Group the arms: $\forall i,j \in \agmgm(0)$ if $\mu_j = \mu_i$, then $i$ and $j$ are grouped. \\
Order the Groups Based on the smallest mean within the group: $G_1, G_2, \dots, G_\ell$. \\ 
Set $p=\ell$
From round $t=1$ to $T$:  \\ 
    \ \ Alternate is pulling arms from group $G_p$. \\ 
    \ \ If the there is an arm in group $p$ that was pulled $\nexit{G_p}$ then set $p=p-1$.
    \ \ Exit if $p=0$. 
\caption{\textsc{Maximize Exit Time: Non-Unique Means}}\label{alg:maximize_exit_non_unique_mean}
\end{algorithm}


\begin{theorem}\label{th:maximize_exit_non_unique_mean}
Algorithm \ref{alg:maximize_exit_non_unique_mean} maximizes the exit time with the means are non-unique.
\end{theorem}
\begin{proof}
The proof follows similar steps to the proof of Theorem \ref{th:max_exit_time_large_gap} with slight differences. Specifically, we first show the following: 
\begin{fact}
The total number of pulls for arms in group $G_i$ can be at most $(\nexit{G_i}-1) |G_i|+1$ before $\mgm(t) \ge \muexit{G_i}$.     
\end{fact}
\begin{proof}
The maximum number of pulls an arm can receive before $\mgm(t) \ge \muexit{G_i}$ is $\nexit{G_i}$ since only one arm can receive $\nexit{G_i}$ pulls and the rest receive $\nexit{G_i}-1$ we have $(\nexit{G_i}-1) \cdot (|G_i|-1) + \nexit{G_i}=(\nexit{G_i}-1) |G_i|+1$. 
\end{proof}
\begin{fact}\label{fact:max_bound_nu}
For any strategy (possibly randomized) followed by the human in any realization we have $\tauexit \leq \sum_{i \in [\ell]} \Big((\nexit{G_i}-1) |G_i|+1 \Big)$.  
\end{fact}
\begin{proof}
In any pull the human can only choose from the set $G_1,\dots,G_{\ell}$ to gain non-negative. Since any arm $i \in G_i$ can be pulled at most $(\nexit{G_i}-1) |G_i|+1$ before the utility becomes negative the above follows.  
\end{proof}
\begin{fact}\label{fact:genmu_below_exit_nu}
For any two groups $g,g'$ with $g>g'$ in the first round where $\max_{i \in g'} \genmu{i} \ge \muexit{g'}$ we have $\max_{i \in g'} \genmu{g'} < \muexit{g}$. 
\end{fact}
\begin{proof}\label{fact:start_over_nu}
This follows by the assumption made in Assumption \ref{assump:seperated_means_or_nonun} above. 
\end{proof}
\begin{fact}
At any round $t$ the algorithm only pulls from the set $\agmgm(t)$ and therefore the per round utility is always non-negative. 
\end{fact}
\begin{proof}
This follows by definition of $\agmgm(t)$ from the previous fact (Fact \ref{fact:genmu_below_exit_nu}).
\end{proof}

\begin{fact}
Each group is pulled $(\nexit{G_i}-1) |G_i|+1$ many times. 
\end{fact}
\begin{proof}
After the first round $t$ where a group $G_i \in [\ell]$ with $i>1$ that has been pulled $(\nexit{G_i}-1) |G_i|+1$ many times for any arm $j \in G_{i-1}$ we have $\genmu{j}(t)=\mu_j - \frac{c}{\sqrt{1+\pullsh{j}(t-1)}}$ with $\pullsh{j}(t-1)=0$. Therefore by Fact \ref{fact:start_over_nu} group $G_{i-1}$ can be pulled $(\nexit{G_{i-1}}-1) |G_{i-1}|+1$ many times.  
\end{proof}
From the above it follows that the total number of rounds is $\sum_{i \in \agmgm(0)} \nexit{i}$ and by Fact \ref{fact:max_bound_nu} is it optimal. 
\end{proof}

\subsection{General Case \SE{Not Solved Yet}}
What if two arms $i,j$ with $\mu_j > \mu_i$: (1) have small differences in the mean such $\mu_i - \frac{c}{1+\nexit{i}} \ge \muexit{j}$. (2) large enough difference in the mean such that $\mu_j - \frac{c}{\sqrt{1+\nexit{i}-1}} = \mu_j - \frac{c}{\sqrt{\nexit{i}}} \ge \muexit{i}$. 

Because of (2) we cannot treat them like groups as in the previous subsection. 


\subsection{What if the Human Follows the Greedy Strategy?} 
Suppose we have the setting where the human follows the greedy strategy of always pulling the best arm, then $\tauexit$ can be in the worst case by about a factor of $K$. To see that suppose that all means are distinct, then following our algorithm we get $\tau=\sum_{i\in [K]} \nexit{i}$ whereas $\tau_{\text{greedy}}=\nexit{1}$. The ratio is the worst case is $\frac{\nexit{1}}{\sum_{i\in [K]} \nexit{i}} \leq \frac{1}{K}$.   



% \begin{algorithm}[h!]
% \caption{\textsc{Maximize Exit Time}}\label{alg:maximize_exit}
%  \begin{algorithmic}
%  \STATE Find $\agmgm(0)$. Let $\barK = |\agmgm(0)|$.
%  \STATE Set $\bar{A}=\agmgm(0)$
%  \FOR{$i = \barK \text{ to } 1$}
%     \STATE Set $G_i = \{j \in \bar{A} | \mu_i -\frac{c}{\sqrt{1+\nexit{i}}}  \ge \muexit{j} \}$. 
%     \STATE Update $\bar{A} = \bar{A} - G_i$.
%     \STATE Update $i=i-(|G_i|-1)$.
%  \ENDFOR 
%  \STATE Re-index the groups to be $G_1, G_2, \dots, G_{\ell}$ 
%  \STATE Set $p=\ell$
%  \STATE From round $t=1$ to $T$: \\    
%     \ \ Alternate is pulling arms from group $G_p$ starting from the smallest mean. \\ 
%     \ \ If the there is an arm in group $p$ that was pulled $\nexit{G_p}$ then set $p=p-1$. \\
%     \ \ Exit if $p=0$. 
% \end{algorithmic} 
% \end{algorithm}


% \begin{theorem}\label{th:maximize_exit}
% Algorithm \ref{alg:maximize_exit} maximizes the exit time.
% \end{theorem}
% \begin{proof}
% The proof is almost identical to the proof of Theorem \ref{th:maximize_exit_non_unique_mean}. Specifically, we first show the following: 
% \begin{fact}
% The total number of pulls for arms in group $G_i$ can be at most $(\nexit{G_i}-1) |G_i|+1$ before $\mgm(t) \ge \muexit{G_i}$.     
% \end{fact}
% \begin{proof}
% The maximum number of pulls an arm can receive before $\mgm(t) \ge \muexit{G_i}$ is $\nexit{G_i}$ since only one arm can receive $\nexit{G_i}$ pulls and the rest receive $\nexit{G_i}-1$ we have $(\nexit{G_i}-1) \cdot (|G_i|-1) + \nexit{G_i}=(\nexit{G_i}-1) |G_i|+1$. 
% \end{proof}
% \begin{fact}\label{fact:max_bound_nu}
% For any strategy (possibly randomized) followed by the human in any realization we have $\tauexit \leq \sum_{i \in [\ell]} \Big((\nexit{G_i}-1) |G_i|+1 \Big)$.  
% \end{fact}
% \begin{proof}
% In any pull the human can only choose from the set $G_1,\dots,G_{\ell}$ to gain non-negative. Since any arm $i \in G_i$ can be pulled at most $(\nexit{G_i}-1) |G_i|+1$ before the utility becomes negative the above follows.  
% \end{proof}
% \begin{fact}\label{fact:genmu_below_exit_nu}
% For any two groups $g,g'$ with $g>g'$ in the first round where $\max_{i \in g'} \genmu{i} \ge \muexit{g'}$ we have $\max_{i \in g'} \genmu{g'} < \muexit{g}$. 
% \end{fact}
% \begin{proof}\label{fact:start_over_nu}
% This follows by the assumption made in Assumption \ref{assump:seperated_means} above. 
% \end{proof}
% \begin{fact}
% At any round $t$ the algorithm only pulls from the set $\agmgm(t)$ and therefore the per round utility is always non-negative. 
% \end{fact}
% \begin{proof}
% This follows by definition of $\agmgm(t)$ from the previous fact (Fact \ref{fact:genmu_below_exit_nu}).
% \end{proof}

% \begin{fact}
% Each group is pulled $(\nexit{G_i}-1) |G_i|+1$ many times. 
% \end{fact}
% \begin{proof}
% After the first round $t$ where a group $G_i \in [\ell]$ with $i>1$ that has been pulled $(\nexit{G_i}-1) |G_i|+1$ many times for any arm $j \in G_{i-1}$ we have $\genmu{j}(t)=\mu_j - \frac{c}{\sqrt{1+\pullsh{j}(t-1)}}$ with $\pullsh{j}(t-1)=0$. Therefore by Fact \ref{fact:start_over_nu} group $G_{i-1}$ can be pulled $(\nexit{G_{i-1}}-1) |G_{i-1}|+1$ many times.  
% \end{proof}
% From the above it follows that the total number of rounds is $\sum_{i \in \agmgm(0)} \nexit{i}$ and by Fact \ref{fact:max_bound_nu} is it optimal. 
% \end{proof}



\subsection{Does this maximize utility as well?}
We show through a counter example that this does not necessarily maximize the utility. Suppose we have two arms such that $\mu_1=1$ and $\mu_2=0.5$ and $\Tilde{\mu}_1=0$ and $\Tilde{\mu}_1=-0.5$. Further, $\probc(1,0)=1$ but $\probc(1,x)= \probc(0.5,x) = \epsilon \ \forall x>0$. The algorithm would would start by pulling arm $2$ but then the entire utility would be at most $\epsilon T$ whereas if the arm pulls arm 1 it would give at least 1.  
\SE{maybe we can still maximize utility with a similar algorithm}

\subsection{Example Where Maximizing $\tauexit$ Maximizes the Utility For the Human} 
Set the choice to: 
\begin{align}
    \probcthresh(\mu_1,\mu_2) = 
        \begin{cases}
            p   &  \text{where constant $p > \rho$ if } \mu_2 < \mu_1-\delta  \\
            < \rho  &  \text{o.w} 
        \end{cases}
\end{align}
The above choice probability is almost like a threshold function giving constant probability $p$ is $\mu_1> \mu_2+\delta$ and otherwise would give some probability below $\rho$ leading to a negative utility. The above also implies that for any arm $i$ we have $\muexit{i} = \mu_i -\delta$. Therefore, to maximize utility we maximize $\tauexit$. Accordingly, we reach the following: 
\begin{theorem}
Suppose the AI follows the strategy $S^*$ of pulling the best generative mean arm $\mgm(t)$ at round $t$ and that the choice probability is $\probcthresh$ then if the the Human follows a strategy $S_{\tau}$ to maximize $\tauexit$ then we have an equilibrium.
\end{theorem}
\begin{proof}
Since the strategy to maximize $\tau$ is oblivious by definition \eqref{eq:tau_exit_def} then it follows that strategy $S^*$ for the AI is a best response strategy by Lemma \ref{lemma:ai_best_resp_obv}. Further, since the choice probability is $\probcthresh$ then utility is maximize by maximizing $\tauexit$. Therefore, $S_{\tau}$ is also a best response and we have an equilibrium. 
\end{proof}


\paragraph{If we have a general utility maximizing algorithm then we can use it to find $\tauexit$:} Simple set $\probc=\probcthresh$ and run the algorithm. 

\subsection{Questions?}
\begin{enumerate}
    \item Maximize $\tau$ for general means? 
    \item How to maximize the utility for general $\probc$? 
    \item What if the horizon is not large?
\end{enumerate}

% \begin{algorithm}[h!]
% Find $A_{\mgm}(0)$.  \\ 
% Group the arms: $\forall i,j \in \arms$ if $\mu_j - \frac{c}{\sqrt{\bar{n}_j}} \ge \mu_i -\delta$, then $i$ and $j$ are grouped. \\ 
% Order the Groups Based on the smallest mean within the group: $G_1, G_2, \dots, G_\ell$. \\ 
% From round $t=1$ to $T$: \\ 
%     Alternate is pulling arms from the smallest group starting from the smallest arm within the group. \\ 
%     \ \ if $\Tilde{\mu}_{\mgm(t)} \ge \mu_i -\delta$ then deactivate $i$ and never pull it again.  
% \caption{\textsc{Maximize Exit Time}}
% \end{algorithm}



==> pausing_is_necessary.tex <==
\subsection{Pausing is Necessary}
Here we will show that if an algorithm does not pause and always plays then it is possible for it to obtain arbitrarily bad utility.


\begin{restatable}{theorem}{pauseth}\label{th:pauseth}
There always exists an instance such that an algorithm that does plays for at least $\alpha T$ of the horizon where the constant $\alpha \in (0,1]$ will receive negative utility and a less than zero multiplicative approximation of the optimal value. 
\end{restatable}


==> short_horizon.tex <==
\clearpage
\newpage 
\section{Short Horizon}
The algorithm we have assume that the horizon is long so what should we do if the horizon is short? 

Define for arm $i$ the following: 
\begin{align}
    \nu_i(\Tilde{\mu}) = \probc(\mu_i,\Tilde{\mu}) - \rho_i 
\end{align}
which the utility at a given value of the generative mean. 

Then suppose the following condition is true: 
\begin{condition}
Given $i,j \in [K]$ then if $i\neq j$ then one of the following is true (by swithching $i$ and $j$): 
\begin{align}
    \text{(1):} \ \ & \nu_i(\Tilde{\mu}) \ge \nu_j(\Tilde{\mu}) \ \ \ \forall  \Tilde{\mu} \\ 
    \text{OR (2):} \ \ \exists \Tilde{\mu}_0, \ \ & \nu_i(\Tilde{\mu}) \ge \nu_j(\Tilde{\mu}) \ \text{if $\Tilde{\mu} \leq \Tilde{\mu}_0$  \ \ and } \ \ \nu_i(\Tilde{\mu}) \leq \nu_j(\Tilde{\mu}) \ \text{if $\Tilde{\mu} \ge \Tilde{\mu}_0$}
\end{align}
\end{condition}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\linewidth]{Pictures/condition.pdf}
    \caption{}
    \label{fig:enter-label}
\end{figure}

\newpage 
How can we use this condition? 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\linewidth]{Pictures/hint.pdf}
    \caption{}
    \label{fig:enter-label}
\end{figure}

==> symbols.tex <==
\section{Symbols}
\begin{table}[h!]
    \centering
    \begin{tabular}{ll}
        Symbol & Meaning \\
        $a_t$ & arm chosen by the AI at round t \\
        $b_t$ & arm chosen by the human at round t  \\
        $\bvec_t$  & human probability vector at round $t$ over the arms\\
        $\avec_t$  & AI probability vector at round $t$ over the arms\\
        $\mu_i$ & ordinary mean of arm $i$ (when pulled by the human)\\
        $\genmu{i}(t)$ & generative mean of arm $i$ (when pulled by the AI) at round $t$\\
        $\pullsh{i}(t)$ & number of times the human has chosen arm $i$ up to and including round $t$\\
        $\pullsuh(t)$ & number of times the user has chosen the human's arm up to and including round $t$\\
        $\pullsuai(t)$ & number of times the user has chosen the AI's arm up to and including round $t$\\
        $c_i$ & cost for pulling arm $i$ incurred by the human\\
        $\mgm(t)= \max\limits_{i \in \arms} \big( \mu_i - g_i(\pullsh{i}(t-1)) \big)$ & the arm with the maximum generative mean at round $t$\\
    \end{tabular}
    \caption{List of symbols and their meanings.}
    \label{tab:my_label}
\end{table}
